Computing Data Distribution from Query Selectivities

We are given a set $\mathcal{Z}=\{(R_1,s_1),\ldots, (R_n,s_n)\}$, where each $R_i$ is a \emph{range} in $\Re^d$, such as rectangle or ball, and $s_i \in [0,1]$ denotes its \emph{selectivity}. The goal is to compute a small-size \emph{discrete data distribution} $\mathcal{D}=\{(q_1,w_1),\ldots, (q_m,w_m)\}$, where $q_j\in \Re^d$ and $w_j\in [0,1]$ for each $1\leq j\leq m$, and $\sum_{1\leq j\leq m}w_j= 1$, such that $\mathcal{D}$ is the most \emph{consistent} with $\mathcal{Z}$, i.e., $\mathrm{err}_p(\mathcal{D},\mathcal{Z})=\frac{1}{n}\sum_{i=1}^n\! \lvert{s_i-\sum_{j=1}^m w_j\cdot 1(q_j\in R_i)}\rvert^p$ is minimized. In a database setting, $\mathcal{Z}$ corresponds to a workload of range queries over some table, together with their observed selectivities (i.e., fraction of tuples returned), and $\mathcal{D}$ can be used as compact model for approximating the data distribution within the table without accessing the underlying contents. In this paper, we obtain both upper and lower bounds for this problem. In particular, we show that the problem of finding the best data distribution from selectivity queries is $\mathsf{NP}$-complete. On the positive side, we describe a Monte Carlo algorithm that constructs, in time $O((n+\delta^{-d})\delta^{-2}\mathop{\mathrm{polylog}})$, a discrete distribution $\tilde{\mathcal{D}}$ of size $O(\delta^{-2})$, such that $\mathrm{err}_p(\tilde{\mathcal{D}},\mathcal{Z})\leq \min_{\mathcal{D}}\mathrm{err}_p(\mathcal{D},\mathcal{Z})+\delta$ (for $p=1,2,\infty$) where the minimum is taken over all discrete distributions. We also establish conditional lower bounds, which strongly indicate the infeasibility of relative approximations as well as removal of the exponential dependency on the dimension for additive approximations. This suggests that significant improvements to our algorithm are unlikely.

==> MWU.tex <==
\section{MWU Algorithm}

For a discrete distribution $\Dist$ and a training set $\TrainingSet$ recall that that $\Error(\Dist, \TrainingSet)=\frac{1}{n}\sum_{i=1}^n|(s_{\Dist}(R_i)-s_i)|$,\\  $OPT=arg\min_{\Dist\in\DistFam}\frac{1}{n}\sum_{i=1}^n|(s_{\Dist}R_i)-s_i)|$, and, $f(|\RangeSet|)$ is a function for the time it takes to compute the weighted deepest point in the arrangement $\Arr(\RangeSet)$. 

\paragraph{Plan} Let $\P=\{p_1,...,p_m\}$  be a finite subset of $\Re^d$ such that it contains exactly one point from each cell in $\Arr(\RangeSet)$. Consider the following optimization problem on $|\P|$ variables where each variable $v_i$ corresponds to the point $p_i\in \P$.

\begin{align*}
\text{minimize} \quad & \frac{1}{n}\sum_{i=1}^n|(\sum_{p_j\in\P\cap R_i}v_j- s_i)| \\
\text{subject to} \quad & \\
& \sum_{p_j\in \P} v_j= 1 \\
& v_j\geq 0 \quad \forall p_j\in \P
\end{align*}

It is easy to see that an optimal solution to the above LP gives an optimal discrete distribution in terms of error. However, computing this can be very expensive as the arrangement may have $\Theta(n^d)$ cells. Our strategy is to solve this optimization problem using the MWU as described in \cite{v008a006} without explicitly constructing all the variables. We note that a straightforward implementation of the MWU method in our problem  also leads to $\Omega(n^d)$ time due to the number of variables. Hence, new ideas are needed to overcome this obstacle.




\subsection{Algorithm}
Let $\alpha \in [0,1]$ be a guess for the optimal error. Let $\eps=\frac{\delta}{16}$.
We discretize the range $[0,1]$ into a list of errors $E=\{\frac{\eps}{2}, (1+\eps)\frac{\eps}{2}, (1+\eps)^2\frac{\eps}{2},\ldots, 1\}$. We guess the optimal error $\alpha$ by running a binary search on $E$.
The algorithm starts with $\alpha$ set to the middle value of $E$ and tries to  find a distribution $\Dist''$ such that $\Error(\Dist'',\TrainingSet)\leq \alpha+\eps$ using MWU.
If it fails, it resets $\alpha$ to a larger value of $E$ following the binary search. If it succeeds, it resets $\alpha$ to a smaller value of $E$ following the binary search. In the end of the binary search, 
for a particular $\alpha$ that the MWU last succeeded, we get $\Dist''$. The algorithm computes an $\eps$-approximation of $\Dist''$ and returns it as the output $\Dist'$.

%If it fails, it resets $\alpha:=\max(1,(1+\eps)\alpha)$ and restarts. For a particular $\alpha$, if the MWU concludes and outputs $\Dist''$, the algorithm computes an $\eps$-approximation of $\Dist''$ and returns it as the output $\Dist'$.
\par In a particular attempt at running MWU, the algorithm tries to iteratively solve the the following optimization problem:
%\paragraph{LP 1}
\begin{align*}
 \\
 \quad & \\
 & \frac{1}{n}\sum_{R_i\in\RangeSet} z_i\leq \alpha \quad \\
& z_i=|\sum_{p_j\in\P\cap R_i}v_j- s_i| \quad \forall R_i\in\RangeSet\\
& v_j\geq 0 \quad \forall p_j\in \P\\
& \sum_{p_j\in \P} v_j\leq 1 \\
& z_i\in [0,1] \quad \forall R_i\in \RangeSet
\end{align*}
The fact that the above optimization problem does not require the sum of the weights to be 1 is not of concern since it is trivial to find a point that lies outside $\RangeSet$ and assign it the remaining mass. Consider the following equivalent LP: 
 \paragraph{LP 2}
\begin{align*}
 \\
 \quad & \\
 & \sum_{R_i\in\RangeSet}-\frac{z_i}{n}\geq -\alpha \quad \text{(Type \RNum{1})} \\
& z_i+\sum_{p_j\in\P\cap R_i}v_j\geq s_i \quad \forall R_i\in\RangeSet \quad \text{(Type \RNum{2})}\\
&  z_i-\sum_{p_j\in\P\cap R_i}v_j\geq -s_i \quad \forall R_i\in\RangeSet \quad \text{(Type \RNum{3})}\\
& \sum_{p_j\in \P} v_j\leq 1 \quad \text{(Type \RNum{4})}\\
& v_j\geq 0 \quad \forall p_j\in \P \quad \text{(Type \RNum{4})}\\
& z_i\in [0,1] \quad \forall R_i\in \RangeSet \quad \text{(Type \RNum{4})}
\end{align*}
In any attempt, the MWU runs for $T=O(\frac{\ln(|\RangeSet|)}{\eps^2})$ iterations. Let $\F$ be a multi-set that is empty initially. In each iteration, the MWU process adds at most one point to $\F$. At the end of $T$ rounds, it returns the discrete distribution with support $\F$ where each point has weight $\frac{1}{T}$.\footnote{Note that the sum of weights of all points may be less than 1.}   Let $\MA\vx\geq \vb$ be the matrix-vector representation of the LP 2 ignoring the Type \RNum{4} constraints. Thus, $\MA$ is the constraint matrix, $\vx$ is the vector representing the variables, and $\vb$ is a vector representing the RHS of the constraints. The MWU algorithm maintains a probability vector $\vp$ whose dimension equals the number of rows of $\MA$. Thus $dim(\vp)=2|\RangeSet|+1$.
Let us denote the coordinate in $\vp$ with respect to the $j$-th Type \RNum{2} (resp. Type \RNum{3}) constraint by $\vpos_j$ (resp. $\vpneg_j$).
Let $Pos$ (resp. $Neg$) be the collection of coordinates of vector $\vp$ with respect to  Type \RNum{2} (resp. Type \RNum{3}) constraints.
%  Let $Pos$ (resp. $Neg$) be the collection of coordinates of the form $\vpos_j$ (resp. $\vpneg_j$).
Note that $|Pos|=|Neg|=|\RangeSet|$. Let $w(Pos)=\sum_{j\in Pos}\vpos_j$ (resp. $w(Neg)=\sum_{j\in Neg}\vpneg_j$) denote the sum of all values in $Pos$ (resp. $Neg$). Initially $\vp$ represents the uniform distribution. In each iteration $t$, the MWU algorithm checks if there exists a solution $\vx^{(t)}$ satisfying all Type \RNum{4} constraints such that $\vp^T\MA\vx^{(t)}\geq \vp^T\vb-\frac{\eps}{2}$ holds.

\paragraph{Checking Feasibility} Consider the expansion of the expression $\vp^T\MA\vx$. Observe that the LHS is of the form $\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{1}{n}C^{-}_i)z_{i}+\sum\limits_{p_j\in\P}(D^{+}_j-D^{-}_j)v_j$ where $C_i^{+}$ and $ D_j^{+}$ (resp. $C_i^{-}$ and $ D_j^{-}$) represent the sum of all positive (resp. negative) coefficients of each $z_i$ and $v_j$ in the expansion of $\vp^T\MA\vx$ respectively.

For any $i\leq |\RangeSet|$, we compute $C_i^+=\vpos_{i}+\vpneg_{i}$. Furthermore, $C_i^-=\vp_1$.
There is no non-trivial type \RNum{4} constraint for variables $z_i$, so for each $z_i^{(t)}$, set $z_i^{(t)}:=0$, if $(C^{+}_i-\frac{1}{n}C^{-}_i)\leq 0$, else set $z_i^{(t)}:=1$. Finally, we set $\gamma_1=\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{1}{n}C^{-}_i)z_{i}^{(t)}$. 


Next, we focus on setting the variables $v_j$, which is a more challenging task because the are $O(n^d)$ of them and there are non-trivial Type \RNum{4} constraints. 
We use an $\eps$-approximation schema to set the variables $v_j$ by (approximately) maximizing $\vp^T\MA\vx$.
We generate a subset of $S_1\subseteq \RangeSet$ by sampling $\kappa=O(\frac{1}{\eps^2}\log |\RangeSet|)$ rectangles where each rectangle $R_j$ is sampled with probability  $\frac{\vpos_j}{w(Pos)}$. Similarly, generate another subset $S_2\subseteq \RangeSet$ by sampling $\kappa$ rectangles where each rectangle $R_j$ is sampled with probability  $\frac{\vpneg_j}{w(Neg)}$. Let $\hat{S}=S_1\cup S_2$ be a weighted set of rectangles where each rectangle in $S_1$ has weight $\frac{w(Pos)}{\kappa}$ and each rectangle in $S_2$ has weight $-\frac{w(Neg)}{\kappa}$. Let $\square$ be the cell in $\Arr(\hat{S})$, the arrangement of $\hat{S}$, of maximum weighted depth. Take an arbitrary point $l_{\square}$ in $\square$.
\newcommand{\indx}{j^{l_\square}}
We find all rectangles in $\RangeSet$ that contain $l_\square$, so we can identify the index $\indx$ such that $p_{\indx}\in \P$ is contained in the same set of rectangles in $\RangeSet$ as the point $l_\square$.
We compute $D^{+}_{\indx}=\sum_{i: p_{\indx}\in R_i}\vpos_{i}$ and $D^{-}_{\indx}=\sum_{i: p_{\indx}\in R_i}\vpneg_{i}$.


If $\gamma+\max(0, (D^{+}_{\indx}-D^{-}_{\indx}))+\frac{\eps}{2}<\vp^T\vb$, declare that the current $\alpha$ is too small and abort the MWU. On the other hand, if $\gamma+max(0,(D^{+}_{\indx}-D^{-}_{\indx}))+\frac{\eps}{2}\geq \vp^T\vb$, then  if $D^{+}_{\indx}-D^{-}_{\indx}>0$, add $l_{\square}$ to $\F$.
%Let $v_{\indx}$ be the variable in LP 2 corresponding to the point $l_{\square}$.
If $(D^{+}_{\indx}-D^{-}_{\indx})>0$, consider $x^{(t)}$ to be the solution determined by setting each $z_i^{(t)}$ as above and ${v_{\indx}^{(t)}=1}$. Else, consider $x^{(t)}$ to be the solution determined by setting each $z_i^{(t)}$ as above and all $v_{\indx}^{(t)}=0$.

Next, the MWU requires to update each coordinate $\vp_j$ of $\vp$ such that ${\vp_j}^{(t+1)}:={\vp_j}^{(t)}\frac{(1-\eta (\MA_j\vx_j^{(t)}-b_j))}{\Phi^{(t)}} $. Depending on the constraint corresponding to $A_i$, the expression $(\MA_j\vx_j-b_j)$ can be determined from the computed values of each $z_i^{(t)}$ in the current iteration as well as checking if the rectangle corresponding to $\vp_j$ contains the point $l_{\square}$. Here $\eta=\frac{\eps}{12}$ and $\Phi^{(t)}$ is a normalizing constant to ensure $\vp$ remains a distribution. After updating $\vp$, the algorithm then moves on to the next iteration.



% Assign an integer label to each constraint in the above LP except for the last two constraints. The MWU algorithm maintains a non-negative weight $\beta_j$ for each constraint with label $j$. Note that there are $2|\RangeSet|+1$ such constraints. In the first iteration, $\forall j$,$B_j:=1$. In a particular iteration, the algorithm checks if the weighted sum of the contraints, where co 



\subsection{Analysis}
\paragraph{Correctness}  Suppose LP 2 has a feasible solution. Observe that for $\forall i\quad |\MA_i\vx-b_i|\in [-2,2]$. Therefore, by Theorem 3.5 of [AroraMWU], if in each iteration of the MWU, the algorithm can find a solution $\vx^{(t)}$ satisfying all Type \RNum{4} constraints such that $\vp^T\MA\vx^{(t)}\geq \vp^T\vb-\frac{\eps}{2}$ holds then after $T=O(\frac{\ln(|\RangeSet|)}{\eps^2})$ iterations, it is true that $\forall i\quad \MA_i\vx\geq \vb_i-\eps$ holds where $\vx=\frac{1}{T}\sum\limits_{t=1}^T \vx^{(t)}$. Assuming the algorithm checks feasibility in each iteration successfully, the description of the algorithm suggests that  $\vx=\frac{1}{T}\sum\limits_{t=1}^T \vx^{(t)}$ is equivalent to the discrete distribution with support $\F$ where each point has weight $\frac{1}{T}$. Because each $z_i$ may not capture the error of $R_i$ exactly, this implies $\Error(\Dist_{\F},\TrainingSet)\leq \Error(OPT,\TrainingSet)+3\eps$. Now it remains to prove that the algorithm can check feasibility in each iteration accurately. 

\par Observe that checking if there exists an $\vx$ such that $\vp^T\MA\vx \geq \vp^T\vb-\frac{\varepsilon}{2}$ under Type $\RNum{4}$ constraints is equivalent to maximizing $\vp^T\MA\vx$ under Type $\RNum{4}$ constraints. Recall that, $\vp^T\MA\vx=\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{1}{n}C^{-}_i)z_{i}+\sum\limits_{p_j\in\P}(D^{+}_j-D^{-}_j)v_j$. Furthermore, note that the two summations can be maximized independently because they do not have common variables. It is easy to verify that the algorithm maximizes $\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{1}{n}C^{-}_i)z_{i}$.
For the term $\sum\limits_{p_j\in\P}(D^{+}_j-D^{+}_j)v_j$, observe that this is maximized by setting the variable with the largest coefficient to one if it is non-negative or else setting everything to zero. This is because $\sum\limits_{p_j\in \P} v_j\leq 1$. Let $v_{j^*}$ denote the variable with the largest coefficient. Recall $v_{\indx}$ is the variable found by the algorithm through the sampling step. 
\begin{lemma}
$(D^{+}_{\indx}-D^{-}_{\indx})\geq (D^{+}_{j^{*}}-D^{-}_{j^*})-\eps $
\end{lemma}
\begin{proof}
Consider the range space $\Sigma=(\Re^d,S_1)$ and its dual $\Sigma^D$. Since $|S_1|=\kappa=O(\frac{1}{\eps^2}\log |\RangeSet|)$, it is known that $S_1$ is an $\frac{\eps}{4}$-approximation for $\Sigma^D$ with probability at least $1-n^{O(d)}$. More specifically, it holds that  $|\frac{w_1(p_{j^*})}{\kappa}- \frac{D^{+}_{j^{*}}}{w(Pos)}|\leq \frac{\eps}{4}$, where $w_1(p_{j^*})$ denotes the  number of rectangles in $S_1$ containing $p_{j^*}$. Similarly, $S_2$ is is an $\frac{\eps}{4}$-approximation for $\Sigma^D$, so it holds that $|\frac{w_2(p_{j^*})}{\kappa}- \frac{D^{-}_{j^{*}}}{w(Neg)}|\leq \frac{\eps}{4}$, where $w_2(p_{j^*})$ denotes the  number of rectangles in $S_2$ containing $p_{j^*}$.
Equivalently, using the fact that $w(Pos)\in [0,1]$ and $w(Neg)\in [0,1]$, we can rewrite the inequalities above as,
$$D_{j^*}^+-\frac{\eps}{4}\leq w_1(p_{j^*})\frac{w(Pos)}{\kappa}\leq D_{j^*}^++\frac{\eps}{4}$$
$$D_{j^*}^--\frac{\eps}{4}\leq w_2(p_{j^*})\frac{w(Neg)}{\kappa}\leq D_{j^*}^-+\frac{\eps}{4},$$
so it follows that,
$$D_{j^*}^+-D_{j^*}^--\frac{\eps}{2}\leq w_1(p_{j^*})\frac{w(Pos)}{\kappa}-w_2(p_{j^*})\frac{w(Neg)}{\kappa}\leq D_{j^*}^+-D_{j^*}^-+\frac{\eps}{2}.$$
The same inequalities hold for any point in $\Re^d$, for example $l_\square$.
Recall that the algorithm chooses a point $l_\square$ in the cell $\square$ of $\Arr(\hat{S})$ with the maximum weighted depth.
By the inequalities above, it holds that,
$$D^{+}_{\indx}-D^{-}_{\indx}\geq w_1(l_\square)\frac{w(Pos)}{\kappa}-w_2(l_\square)\frac{w(Neg)}{\kappa}-\frac{\eps}{2}\geq w_1(p_{j^*})\frac{w(Pos)}{\kappa}-w_2(p_{j^*})\frac{w(Neg)}{\kappa}-\frac{\eps}{2}\geq D_{j^*}^+-D_{j^*}^--\eps.$$


%Together, they imply that for any point lying in a particular cell $\Delta$ of $\Arr(\hat{S}=S_1\cup S_2)$  (where each rectangle in $S_1$ has weight $\frac{w(Pos)}{\kappa}$ and each rectangle in $S_2$ has weight $-\frac{w(Neg)}{\kappa}$) the coefficient of its corresponding variable in $\vp^T\MA\vx$ is within $\frac{\eps}{4}$ of the weight of $\Delta$ in $\Arr(\hat{S})$. In particular this implies $v_{\indx}$ has coefficient at least $D^{+}_{j^{*}}-D^{-}_{j^{*}}-\frac{\eps}{2}$. 

\end{proof}

In any iteration of the MWU for $\alpha\geq \Error(OPT,\TrainingSet)$
%$\alpha\in [\max(\frac{\eps}{2}, \Error(OPT,\TrainingSet)),\max(\frac{\eps}{2}, (1+\eps)\Error(OPT,\TrainingSet))]$,
there exists a feasible solution, and therefore $max(0,D^{+}_{j^{*}}-D^{-}_{j^{*}})\geq\vp^T\vb-\gamma $. The above lemma implies $max(0,D^{+}_{j^{*}}-D^{-}_{j^{*}})-\max(0, (D^{+}_{\indx}-D^{-}_{\indx}) )\leq \frac{\eps}{2}$. Therefore, $\gamma+\max(0, w(l_{\square}))+\frac{\eps}{2}\geq \vp^T\vb$ must hold. This concludes the proof that the algorithm always finds a feasible solution when $\alpha$ in the above range.
\par Combining above along with the fact that the algorithm take an $\eps$-approximation (recall $\eps=\frac{\delta}{16}$)  at the end implies, $|\Dist'|\leq O(\frac{1}{\delta^2}\log\frac{1}{\delta})$ and $\Error(\Dist',\TrainingSet)\leq \Error(OPT,\TrainingSet)+\delta$ with high probability. 
\paragraph{Running Time}
The size of $E$ is $O(\frac{1}{\eps}\log\frac{1}{\eps})$ so the algorithm requires $O(\log\frac{1}{\eps}+\log\log\frac{1}{\eps})$ attempts.
%Since the algorithm starts with $\alpha=\frac{\eps}{2}$ and increases $\alpha$ by a factor of $(1+\eps)$ in each new attempt, it requires $O(\frac{1}{\eps}\log \frac{1}{\eps})$ attempts.
In each iteration of MWU, the coefficients of all the $z_i$ along with $\gamma$ can be computed in $O(n)$ time. Sampling $S_1$ and $S_2$ also require $O(n)$ time. Computing a point in the deepest cell of $\Arr(\hat{S})$ requires $f(|hat{S}|)=f(\frac{1}{\eps^2}\log |\RangeSet|)$.
Identifying the cell $p_{\indx}$ and computing the coefficient for the required $v_{\indx}$ variable takes $O(n)$ time. Each attempt of the MWU requires at most $\frac{1}{\eps^2}\log |\RangeSet|$ iterations. Since $\eps=\frac{\delta}{16}$, the overall running time is $O((\log\frac{1}{\delta}+\log\log \frac{1}{\delta})(n+f(\frac{1}{\delta^2}\log^{\frac{d}{2}} |\RangeSet|))\frac{1}{\delta^2}\log |\RangeSet|)$.

If $\RangeSet$ consists of a set of rectangles then the deepest cell of $\Arr(\hat{S})$ can be computed in
$\Tilde{O}(|\hat{S}|^{d/2})=\Tilde{O}(\frac{1}{\eps^d}\log^{\frac{d}{2}} |\RangeSet|)$ time using standard techniques \cite{oy-nubkm-91}. The overall running time is $\Tilde{O}((\log\frac{1}{\delta}+\log\log \frac{1}{\delta})(n+\frac{1}{\delta^d}\log^{\frac{d}{2}} |\RangeSet|)\frac{1}{\delta^2}\log |\RangeSet|)=\tilde{O}(\frac{n}{\delta^2}+\frac{1}{\delta^{d+2}})$.

==> Misc/MWU_new.tex <==






\section{Algorithm}

% A range space $=(\GroundSet,\RangeSet)$ comprises a set of objects $\GroundSet$ and a collection of subsets $\RangeSet$. For instance, $\GroundSet=\Re^d$ and $\RangeSet$ could be the set of all $d$-dimensional rectangles, or balls, or half-spaces. Let $\Dist$ denote a probability distribution over $\GroundSet$. Then, the \emph{selectivity} of a range $R\in \RangeSet$ with respect to $\Dist$, denoted $s_{\Dist}(R)$, is defined as $s_{\Dist}(R):=\Pr_{x\sim \Dist}[x\in R]$. 
 
 
\par Let $\TrainingSet=\{z_1,...,z_n\}$ be a set of training samples where each $z_i=(R_i,s_i)\in \RangeSet\times[0,1]$ i.e. a range and its selectivity. The goal here is to find a $\Dist\in\mathbb{D}$ that minimizes the expected loss function  i.e.
\begin{equation*}
\min_{\Dist\in\DistFam} \Error(\Dist, \TrainingSet) = \min_{\Dist\in\DistFam} \frac{1}{n}\sum_{i=1}^n \left(s_{\Dist}(R_i) - s_i\right)^2
\end{equation*}

Let $\opt:= \min_{\Dist\in\DistFam} \Error(\Dist, \TrainingSet)$. In this paper, we design an efficient algorithm that finds a discrete distribution of small size whose error with respect to $\TrainingSet$ is close to $\opt$. We demonstrate an algorithm which reduces this task to polylogarithmic computations of the deepest point with respect to a small set of weighted ranges. Before presenting the main result we need a few definitions.

\par Let  $\RangeSet$ be a set of ranges and  $w:\RangeSet\rightarrow \Re$ a weight function (weights can be both positive and negative). The \emph{depth} of a point $p\in \Re^d$ with respect to $(\RangeSet,w)$ is defined to be $\depth(p)=\sum_{R\in \RangeSet} \mathbf{1}(p\in R)w(R) $

Let $\alg$ be an algorithm that given a set of weighted ranges $(\RangeSet,w)$  finds a deepest point i.e. $\alg(\RangeSet,w)$ returns a point $\hat{p}$ such that $depth(\hat{p})= \max_{p\in \Re^d} \sum_{R\in \RangeSet} \mathbf{1}(p\in R)w(R)$. Let the running time of $\alg$ be defined by the function $T(|\RangeSet|)$.

The main theorem we prove in this section is the following.

\begin{theorem}
Let $\TrainingSet=\{z_1,...,z_n\}$ be a set of training samples where each $z_i=(R_i,s_i)\in \RangeSet\times[0,1]$, and a parameter $\delta\in (0,1)$.
There exists an algorithm that returns a discrete distribution $\Dist'$ of size $|\Dist'|=O(\frac{\log n}{\delta^2}\log\frac{1}{\delta})$ such that $\Error(\Dist',\TrainingSet)\leq \Error(\opt,\TrainingSet)+\delta$ with high probability. Furthermore, the algorithm takes $O(\frac{n \log n}{\delta^2}+T(\frac{\log n}{\delta^2})\frac{\log n}{\delta})$ time. 
\end{theorem}
 






% \subsection{Algorithm2}
% Let $\iter=??$. Suppose $\alpha\geq \opt$ and $\delta\in [0,1]$. Our goal is to solve the following optimization problem.

% \begin{align*}
%  \\
%  \quad & \\
%  & \frac{1}{n}\sum_{R_i\in\RangeSet} z_i^2\leq \alpha+\delta \quad \quad \text{(Type 0)} \\
% & z_i\geq s_D(R_i)-s_i \quad \forall R_i\in\RangeSet \quad \text{(Type \RNum{1})} \\
% & z_i \geq s_i-s_D(R_i) \quad \forall R_i\in\RangeSet \text{(Type \RNum{2})} \\
% & \Dist'\in \DistFam_{\iter} 
% \end{align*}

% As long as $\alpha\geq \opt$, the above always has a feasible solution because $\Dist'$ can always be considered to be a $\frac{\delta}{2}$-approximation of $\arg\min_{\Dist\in\DistFam} \Error(\Dist,\TrainingSet)$ which always has size $O(\iter)$. Of course, to compute such an approximation we would need access to $\arg\min_{\Dist\in\DistFam} \Error(\Dist,\TrainingSet)$ which we do not have. Instead, we will attempt to solve this optimization problem using the MWU algorithm in Section ?. Our approach is in line with prior work using MWU to solve optimization problems. See PST and AHK.
% \par Consider an instantiation of the MWU framework in Section ?.


% \begin{itemize}
%     \item Decisions: Let there be $2n+1$ decisions, one corresponding to each constraint of the above optimization problem.

%     \item Weights: Recall that the MWU also stores a weight corresponding to each decision which is updated after every iteration. We will store these weights in an array $\W$ of size $2n+1$. Let us assume that $\W$ is indexed starting from $0$. It will be convenient to split $W$ into three subsets: $\{W[0]\}$, $\Pos=\{W[1],...,W[n]\}$ and $\Neg=\{W[n+1],...,W[2n]\}$. We use $\Pos[i]$ (resp. $\Neg[i]$) to refer to $\W[i]$ (resp. $\W[n+i]$). Essentially, $\W[0]$ stores the weight corresponding to the sole Type 0 constraint, whereas $\Pos[i]$ (resp. $\Neg[i]$) stores the weight of the Type 1 (resp. Type 2) constraint corresponding to range $R_i$. Initially, $\W[i]=1$ for all $i\in \{0,...,2n\}$

%     \item Error: In each iteration,  Let the the error for decision $i\in \{0,...,2n\}$


    
% \end{itemize}





% \par  The MWU algorithm runs for $\iter=O(?)$. In each iteration, it adds at most one new point to a set $\F$. Initially, $\F=\emptyset$. If it successfully completes $\iter$ iterations it returns $\F$ assigning each point a weight of $\frac{1}{\iter}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Algorithm L2}

 Let $\alpha \in [0,1]$ be a guess for the optimal error. Let $\eps=\frac{\delta}{16}$.
We discretize the range $[0,1]$ into a list of errors $E=\{\frac{\eps}{2}, (1+\eps)\frac{\eps}{2}, (1+\eps)^2\frac{\eps}{2},\ldots, 1\}$. We guess the optimal error $\alpha$ by running a binary search on $E$.
The algorithm starts with $\alpha$ set to the middle value of $E$ and tries to  find a distribution $\Dist'$ such that $\Error(\Dist',\TrainingSet)\leq \alpha+\eps$ using \solver (details specified below).
If it fails, it resets $\alpha$ to a larger value of $E$ following the binary search. If it succeeds, it resets $\alpha$ to a smaller value of $E$ following the binary search. In the end of the binary search, for a particular $\alpha$ that \solver last succeeded, we get $\Dist'$.

\paragraph{\solver}

% \textcolor{red}{Rahul: Maybe we shouldn't call this MWU and come up with a different name}  

In a particular run of \solver, the goal is to find a discrete distribution with support size at most $\iter=O(\frac{\ln(n)}{\delta^2})$ that satisifes the following constraints:
%\paragraph{LP 1}
\begin{align*}
 \\
 \quad & \\
 & \frac{1}{n}\sum_{R_i\in\RangeSet} z_i^2\leq \alpha+\delta \quad \quad  \\
& z_i\geq s_D(R_i)-s_i \quad \forall R_i\in\RangeSet \quad  \\
& z_i \geq s_i-s_D(R_i) \quad \forall R_i\in\RangeSet  \\
& \Dist'\in \DistFam_{\iter}
\end{align*}

As long as $\alpha\geq \opt$, this is always possible because $\Dist'$ can always be taken to be a $\delta$-approximation of $\arg\min_{\Dist\in\DistFam} \Error(\Dist,\TrainingSet)$ whose size is bounded by $\iter$. Of course, there is no obvious way to compute it directly as we do not have access to $\arg\min_{\Dist\in\DistFam} \Error(\Dist,\TrainingSet)$.
\par In order to find a discrete distribution satifying these constraints, we will use the MWU algorithm from Subsection~\ref{subsec:MWU}. It will be convenient for us to reformulate the above constraints as follows: 

\par Let $\P=\{p_1,...,p_m\}$  be a finite subset of $\Re^d$ such that it contains exactly one point from each cell in $\Arr(\RangeSet)$. Consider the following optimization problem on $|\P|$ variables where each variable $v_i$ corresponds to the point $p_i\in \P$.
\paragraph{Feasibility Problem (FP)}
\begin{align*}
 \\
 \quad & \\
 & \sum_{R_i\in\RangeSet}-\frac{z_i^2}{n}\geq -\alpha \quad \text{(Type \RNum{1})} \\
& z_i+\sum_{p_j\in\P\cap R_i}v_j\geq s_i \quad \forall R_i\in\RangeSet \quad \text{(Type \RNum{2})}\\
&  z_i-\sum_{p_j\in\P\cap R_i}v_j\geq -s_i \quad \forall R_i\in\RangeSet \quad \text{(Type \RNum{3})}\\
& \sum_{p_j\in \P} v_j\leq 1 \quad \text{(Type \RNum{4})}\\
& v_j\geq 0 \quad \forall p_j\in \P \quad \text{(Type \RNum{4})}\\
& z_i\in [0,1] \quad \forall R_i\in \RangeSet \quad \text{(Type \RNum{4})}
\end{align*}

Any discrete distribution can always be mapped to points in $\Arr(\RangeSet)$, hence it is easy to see that an optimal solution to the above constraints gives an optimal discrete distribution in terms of error. 
% Here, the Type \RNum{2} and Type \RNum{3} constraints capture the error of each range whereas the Type \RNum{1} constraint ensures the overall quality of the solution.  
Furthermore, it can be verified that each constraint in \FP is concave. Hence, the MWU algorithm from Subsection~\ref{subsec:MWU} can be applied to solve \FP. However, there is a major issue: The feasibility problem has too many variables as the arrangement may have $\Theta(n^d)$ cells. Moreover, the constraints do not ensure that the size of the discrete distribution is bounded by $\iter$. 
Hence, to get near-linear time, new ideas are needed to overcome these obstacles.  Our high-level strategy is to solve \FP using  MWU implicitly i.e. without explicitly constructing all the variables. Next, we describe the details of \solver. In the analysis we will discuss how the operations performed by \solver map to the MWU algorithm.

\par  Let $\F$ be a multi-set that is empty initially. \solver works iteratively and runs for at most $\iter$ iterations. At the end of each iteration, it adds at most one point to $\F$. If it successfully completes $\iter$ rounds, it returns the discrete distribution with support $\F$ where each point has weight $\frac{1}{\iter}$. 


  \par Let the sole Type \RNum{1} constraint be represented by the function $\cons$. Let the Type \RNum{2} (resp. Type \RNum{3}) constraint with respect to $R_i$ be represented by the function $\cons_i^+$ (resp. $\cons_i^-$). Let $\vx$ be the vector representing the variables, and $\vb$ is a vector representing the RHS of the constraints. \solver also maintains a probability vector $\vp$ whose dimension equals the number of constraints. Thus $dim(\vp)=2|\RangeSet|+1$. Let $\vp_0$ denote the coordinate in $\vp$ with respect to the Type \RNum{1} constraint. Let us denote the coordinate in $\vp$ with respect to $\cons^+$ (resp. $\cons^-$) constraint by $\vpos_j$ (resp. $\vpneg_j$).
Let $Pos$ (resp. $Neg$) be the collection of coordinates of vector $\vp$ with respect to  Type \RNum{2} (resp. Type \RNum{3}) constraints. Note that $|Pos|=|Neg|=|\RangeSet|$. Let $w(Pos)=\sum_{j\in Pos}\vpos_j$ (resp. $w(Neg)=\sum_{j\in Neg}\vpneg_j$) denote the sum of all values in $Pos$ (resp. $Neg$). \solver initially sets $\vp$ to equal the all-ones vector. It then runs for $\iter=O(\frac{\ln(|\RangeSet|)}{\eps^2})$ iterations. In each iteration $t$, \solver checks if there exists a solution $\vx^{(t)}$ satisfying all Type \RNum{4} constraints such that $\vp_0\cons(\vx)+\sum\limits_{i=1}^n \vp_i^+\cons^{+}(\vx)+\sum\limits_{i=1}^n \vp_i^-\cons^{-}(\vx)\geq \vp^T \vb-\frac{\eps}{2}$. 








% \par Let $\MA\vx\geq \vb$ be the matrix-vector representation of the LP 2 ignoring the Type \RNum{4} constraints. Thus, $\MA$ is the constraint matrix, $\vx$ is the vector representing the variables, and $\vb$ is a vector representing the RHS of the constraints. The MWU algorithm maintains a probability vector $\vp$ whose dimension equals the number of rows of $\MA$. Thus $dim(\vp)=2|\RangeSet|+1$.
% Let us denote the coordinate in $\vp$ with respect to the $j$-th Type \RNum{2} (resp. Type \RNum{3}) constraint by $\vpos_j$ (resp. $\vpneg_j$).
% Let $Pos$ (resp. $Neg$) be the collection of coordinates of vector $\vp$ with respect to  Type \RNum{2} (resp. Type \RNum{3}) constraints.
% %  Let $Pos$ (resp. $Neg$) be the collection of coordinates of the form $\vpos_j$ (resp. $\vpneg_j$).
% Note that $|Pos|=|Neg|=|\RangeSet|$. Let $w(Pos)=\sum_{j\in Pos}\vpos_j$ (resp. $w(Neg)=\sum_{j\in Neg}\vpneg_j$) denote the sum of all values in $Pos$ (resp. $Neg$). Initially $\vp$ represents the uniform distribution. In each iteration $t$, the MWU algorithm checks if there exists a solution $\vx^{(t)}$ satisfying all Type \RNum{4} constraints such that $\vp^T\MA\vx^{(t)}\geq \vp^T\vb-\frac{\eps}{2}$ holds.

\paragraph{Checking Feasibility} In order to check the feasibility, it is sufficient to find $\vx$ that maximizes $\vp_0\cons(\vx)+\sum\limits_{i=1}^n \vp_i^+\cons^{+}(\vx)+\sum\limits_{i=1}^n \vp_i^-\cons^{-}(\vx)$ under Type $\RNum{4}$ constraints. We consider the expansion of this expression. Observe that it is is of the form $\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{z_i}{n}C^{-}_i)z_{i}+\sum\limits_{p_j\in\P}(D^{+}_j-D^{-}_j)v_j$ where $C_i^{+}$ and $ D_j^{+}$ (resp. $C_i^{-}$ and $ D_j^{-}$) represent the sum of all positive (resp. negative) coefficients of each $z_i$ and $v_j$ in the expansion of $\vp_0\cons(\vx)+\sum\limits_{i=1}^n \vp_i^+\cons^{+}(\vx)+\sum\limits_{i=1}^n \vp_i^-\cons^{-}(\vx)$ respectively.

For any $i\leq |\RangeSet|$, we have $C_i^+=\vpos_{i}+\vpneg_{i}$. Furthermore, $C_i^-=\vp_0$.
There is no non-trivial type \RNum{4} constraint for variables $z_i$, so using calculus we get $z_i^{(t)}=\min\left\{1, \frac{nC_i^+}{2C_i^-}\right\}$.
%for each $z_i^{(t)}$ set,  
%\begin{enumerate}
%    \item $z_i=1$ if  $\frac{C_i^-}{2nC_i^+} < 0$
%    \item  $z_i=0$ if  $\frac{C_i^-}{2nC_i^+} > 1$
%    \item $z_i=\frac{C_i^-}{2nC_i^+}$ if  $0 \leq \frac{C_i^-}{2nC_i^+} \leq 1$
%\end{enumerate}
Finally, we set $\gamma_1=\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{1}{n}C^{-}_i)z_{i}^{(t)}$. 


Next, we focus on setting the variables $v_j$, which is a more challenging task because the are $O(n^d)$ of them and there are non-trivial Type \RNum{4} constraints. 
We use an $\eps$-approximation schema to set the variables $v_j$ that (approximately) maximizes $\sum\limits_{i=1}^n \vp_i^+\cons^{+}(\vx)+\sum\limits_{i=1}^n \vp_i^-\cons^{-}(\vx)$.
\par First, we generate a subset of $S_1\subseteq \RangeSet$ by sampling $\kappa=O(\frac{1}{\eps^2}\log \log n)$ rectangles where each rectangle $R_j$ is sampled with probability  $\frac{\vpos_j}{w(Pos)}$. Similarly, generate another subset $S_2\subseteq \RangeSet$ by sampling $\kappa$ rectangles where each rectangle $R_j$ is sampled with probability  $\frac{\vpneg_j}{w(Neg)}$. Let $\hat{S}=S_1\cup S_2$ be a weighted set (possibly multi-set) of rectangles. Let $w:\hat{S}\rightarrow \Re$ be a weight function such that $w(s)=\frac{w(Pos)}{\kappa}$ if $s\in S_1$ else $w(s)=-\frac{w(Neg)}{\kappa}$. Let $\square$ be the cell in $\Arr(\hat{S})$, the arrangement of $\hat{S}$, of maximum weighted depth.  Run $\alg(\hat{S},w)$ to find an arbitrary point $l_{\square}$ in $\square$.
\newcommand{\indx}{j^{l_\square}}
We find all rectangles in $\RangeSet$ that contain $l_\square$, so we can identify the index $\indx$ such that $p_{\indx}\in \P$ is contained in the same set of rectangles in $\RangeSet$ as the point $l_\square$.
We compute $D^{+}_{\indx}=\sum_{i: p_{\indx}\in R_i}\vpos_{i}$ and $D^{-}_{\indx}=\sum_{i: p_{\indx}\in R_i}\vpneg_{i}$. If $\gamma+\max(0, (D^{+}_{\indx}-D^{-}_{\indx}))+\frac{\eps}{2}<\vp^T\vb$, % we restart if the number of attempts is fewer than $O(\log n)$, 
 we declare that the current $\alpha$ is too small and abort \solver. 
\par On the other hand, if $\gamma+max(0,(D^{+}_{\indx}-D^{-}_{\indx}))+\frac{\eps}{2}\geq \vp^T\vb$, then  if $D^{+}_{\indx}-D^{-}_{\indx}>0$, add $l_{\square}$ to $\F$.
%Let $v_{\indx}$ be the variable in LP 2 corresponding to the point $l_{\square}$.
If $(D^{+}_{\indx}-D^{-}_{\indx})>0$, consider $x^{(t)}$ to be the solution determined by setting each $z_i^{(t)}$ as above and ${v_{\indx}^{(t)}=1}$. Else, consider $x^{(t)}$ to be the solution determined by setting each $z_i^{(t)}$ as above and all $v_{\indx}^{(t)}=0$.

\paragraph{Updating Weights} Next, \solver updates each coordinate $\vp_j$ of $\vp$ such that ${\vp_j}^{(t+1)}:={\vp_j}^{(t)}\frac{(1-\eta (\cons_j(\vx_j^{(t)})-b_j))}{\Phi^{(t)}} $. Depending on the constraint corresponding to $\cons_i$, the expression $(\cons_j(\vx_j)-b_j)$ can be determined from the computed values of each $z_i^{(t)}$ in the current iteration as well as checking if the rectangle corresponding to $\vp_j$ contains the point $l_{\square}$. Here $\eta=\frac{\eps}{12}$ and $\Phi^{(t)}$ is a normalizing constant to ensure $\vp$ remains a distribution. After updating $\vp$, \solver then moves on to the next iteration.



% Assign an integer label to each constraint in the above LP except for the last two constraints. The MWU algorithm maintains a non-negative weight $\beta_j$ for each constraint with label $j$. Note that there are $2|\RangeSet|+1$ such constraints. In the first iteration, $\forall j$,$B_j:=1$. In a particular iteration, the algorithm checks if the weighted sum of the contraints, where co 



\subsection{Analysis}
\paragraph{Correctness}  It is easy to see that \solver emulates MWU. Suppose \FP has a feasible solution. Observe that for $\forall i\quad |\cons_i(\vx)-b_i|\in [-2,2]$. Therefore, by Theorem~\ref{thm:MWU}, if in each iteration $t$ of \solver, it finds a solution $\vx^{(t)}$ satisfying all Type \RNum{4} constraints such that $\vp_0\cons(\vx)+\sum\limits_{i=1}^n \vp_i^+\cons^{+}(\vx)+\sum\limits_{i=1}^n \vp_i^-\cons^{-}(\vx)\geq \vp^T \vb-\frac{\eps}{2}$, then after $\iter=O(\frac{\ln(|\RangeSet|)}{\eps^2})$ iterations, it is true that $\forall i\quad \cons_i(\vx)\geq \vb_i-\eps$ holds where $\vx=\frac{1}{T}\sum\limits_{t=1}^T \vx^{(t)}$. Assuming the algorithm checks feasibility in each iteration successfully, the description of the algorithm suggests that  $\vx=\frac{1}{T}\sum\limits_{t=1}^T \vx^{(t)}$ is equivalent to the discrete distribution with support $\F$ where each point has weight $\frac{1}{T}$. Because each $z_i$ may not capture the error of $R_i$ exactly, this implies $\Error(\Dist_{\F},\TrainingSet)\leq \Error(OPT,\TrainingSet)+3\eps$. Now it remains to prove that the algorithm can check feasibility in each iteration accurately. 

\par Observe that checking if there exists an $\vx$ such that $\vp_0\cons(\vx)+\sum\limits_{i=1}^n \vp_i^+\cons^{+}(\vx)+\sum\limits_{i=1}^n \vp_i^-\cons^{-}(\vx)\geq \vp^T \vb-\frac{\eps}{2}$ under Type $\RNum{4}$ constraints is equivalent to maximizing $\vp_0\cons(\vx)+\sum\limits_{i=1}^n \vp_i^+\cons^{+}(\vx)+\sum\limits_{i=1}^n \vp_i^-\cons^{-}(\vx)$ under Type $\RNum{4}$ constraints. Recall that, $\vp_0\cons(\vx)+\sum\limits_{i=1}^n \vp_i^+\cons^{+}(\vx)+\sum\limits_{i=1}^n \vp_i^-\cons^{-}(\vx)=\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{z_{i}}{n}C^{-}_i)z_{i}+\sum\limits_{p_j\in\P}(D^{+}_j-D^{-}_j)v_j$. Furthermore, note that the two summations can be maximized independently because they do not have common variables. 
%%%%%%%%%%%
\begin{lemma}


Let $f(x) = C_i^+ x^2 - \frac{C_i^-}{n} x$ be a quadratic function defined on the interval $[0,1]$. The maximum of this function on the given interval can be determined as follows:

First, compute the derivative of the function: $f'(x) = 2C_i^+ x - \frac{C_i^-}{n}$.

Then, solve for $x$ in the equation $f'(x) = 0$, which gives a critical point: $x = \frac{\frac{C_i^-}{n}}{2 C_i^+} = \frac{C_i^-}{2nC_i^+}$.

The maximum of $f(x)$ on the interval $[0,1]$ is obtained at:

\begin{enumerate}
    \item The endpoint $x = 1$, if $\frac{C_i^-}{2nC_i^+} < 0$.
    \item The critical point $x = \frac{C_i^-}{2nC_i^+}$, if $0 \leq \frac{C_i^-}{2nC_i^+} \leq 1$.
    \item The endpoint $x = 0$, if $\frac{C_i^-}{2nC_i^+} > 1$.
\end{enumerate}

Finally, substitute these $x$ values back into the original function $f(x)$ to obtain the corresponding $y$ values, which are the maximum values of the function on the interval $[0,1]$.
\end{lemma}


%%%%%%%%
Thus, \solver maximizes $\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{1}{n}C^{-}_i)z_{i}$ for each $z$.
For the term $\sum\limits_{p_j\in\P}(D^{+}_j-D^{+}_j)v_j$, observe that this is maximized by setting the variable with the largest coefficient to one if it is non-negative or else setting everything to zero. This is because $\sum\limits_{p_j\in \P} v_j\leq 1$. Let $v_{j^*}$ denote the variable with the largest coefficient.
Observe that finding $v_{j^*}$ is equivalent to finding the deepest point in $(\RangeSet,w)$ 
where $w$ is a weight function such that $w(R_i)=\vp^{+}_i-\vp^{+}_i$. However, computing the deepest point is $W[1]$-hard for certain range spaces. Hence, \solver uses sampling to find the approximate deepest point.


Recall $v_{\indx}$ is the variable found by the algorithm through the sampling step. 
\begin{lemma}
$(D^{+}_{\indx}-D^{-}_{\indx})\geq (D^{+}_{j^{*}}-D^{-}_{j^*})-\eps $
\end{lemma}
\begin{proof}
Consider the range space $\Sigma=(\Re^d,S_1)$ and its dual $\Sigma^D$. Since $|S_1|=\kappa=O(\frac{1}{\eps^2}\log |\RangeSet|)$, it is known that $S_1$ is an $\frac{\eps}{4}$-approximation for $\Sigma^D$ with probability at least $\frac{1}{100}$. More specifically, it holds that  $|\frac{w_1(p_{j^*})}{\kappa}- \frac{D^{+}_{j^{*}}}{w(Pos)}|\leq \frac{\eps}{4}$, where $w_1(p_{j^*})$ denotes the  number of rectangles in $S_1$ containing $p_{j^*}$. Similarly, $S_2$ is is an $\frac{\eps}{4}$-approximation for $\Sigma^D$, so it holds that $|\frac{w_2(p_{j^*})}{\kappa}- \frac{D^{-}_{j^{*}}}{w(Neg)}|\leq \frac{\eps}{4}$, where $w_2(p_{j^*})$ denotes the  number of rectangles in $S_2$ containing $p_{j^*}$.
Equivalently, using the fact that $w(Pos)\in [0,1]$ and $w(Neg)\in [0,1]$, we can rewrite the inequalities above as,
$$D_{j^*}^+-\frac{\eps}{4}\leq w_1(p_{j^*})\frac{w(Pos)}{\kappa}\leq D_{j^*}^++\frac{\eps}{4}$$
$$D_{j^*}^--\frac{\eps}{4}\leq w_2(p_{j^*})\frac{w(Neg)}{\kappa}\leq D_{j^*}^-+\frac{\eps}{4},$$
so it follows that,
$$D_{j^*}^+-D_{j^*}^--\frac{\eps}{2}\leq w_1(p_{j^*})\frac{w(Pos)}{\kappa}-w_2(p_{j^*})\frac{w(Neg)}{\kappa}\leq D_{j^*}^+-D_{j^*}^-+\frac{\eps}{2}.$$
The same inequalities hold for any point in $\Re^d$, for example $l_\square$.
Recall that the algorithm chooses a point $l_\square$ in the cell $\square$ of $\Arr(\hat{S})$ with the maximum weighted depth.
By the inequalities above, it holds that,
$$D^{+}_{\indx}-D^{-}_{\indx}\geq w_1(l_\square)\frac{w(Pos)}{\kappa}-w_2(l_\square)\frac{w(Neg)}{\kappa}-\frac{\eps}{2}\geq w_1(p_{j^*})\frac{w(Pos)}{\kappa}-w_2(p_{j^*})\frac{w(Neg)}{\kappa}-\frac{\eps}{2}\geq D_{j^*}^+-D_{j^*}^--\eps.$$


%Together, they imply that for any point lying in a particular cell $\Delta$ of $\Arr(\hat{S}=S_1\cup S_2)$  (where each rectangle in $S_1$ has weight $\frac{w(Pos)}{\kappa}$ and each rectangle in $S_2$ has weight $-\frac{w(Neg)}{\kappa}$) the coefficient of its corresponding variable in $\vp^T\MA\vx$ is within $\frac{\eps}{4}$ of the weight of $\Delta$ in $\Arr(\hat{S})$. In particular this implies $v_{\indx}$ has coefficient at least $D^{+}_{j^{*}}-D^{-}_{j^{*}}-\frac{\eps}{2}$. 

\end{proof}

In any iteration of the MWU for $\alpha\geq \Error(OPT,\TrainingSet)$
%$\alpha\in [\max(\frac{\eps}{2}, \Error(OPT,\TrainingSet)),\max(\frac{\eps}{2}, (1+\eps)\Error(OPT,\TrainingSet))]$,
there exists a feasible solution, and therefore $max(0,D^{+}_{j^{*}}-D^{-}_{j^{*}})\geq\vp^T\vb-\gamma $. The above lemma implies $max(0,D^{+}_{j^{*}}-D^{-}_{j^{*}})-\max(0, (D^{+}_{\indx}-D^{-}_{\indx}) )\leq \frac{\eps}{2}$. Therefore, $\gamma+\max(0, w(l_{\square}))+\frac{\eps}{2}\geq \vp^T\vb$ must hold. Given that these steps are repeated up to $O(\log n)$ times, this concludes the proof that the algorithm always finds a feasible solution when $\alpha$ in the above range with high probability.
% \par Combining above along with the fact that the algorithm take an $\eps$-approximation (recall $\eps=\frac{\delta}{16}$)  at the end implies, $|\Dist'|\leq O(\frac{1}{\delta^2}\log\frac{1}{\delta})$ and $\Error(\Dist',\TrainingSet)\leq \Error(OPT,\TrainingSet)+\delta$ with high probability. 
\paragraph{Running Time}
The size of $E$ is $O(\frac{1}{\eps}\log\frac{1}{\eps})$ so the algorithm requires $O(\log\frac{1}{\eps}+\log\log\frac{1}{\eps})$ attempts.
%Since the algorithm starts with $\alpha=\frac{\eps}{2}$ and increases $\alpha$ by a factor of $(1+\eps)$ in each new attempt, it requires $O(\frac{1}{\eps}\log \frac{1}{\eps})$ attempts.
In each iteration of MWU, the coefficients of all the $z_i$ along with $\gamma$ can be computed in $O(n)$ time. Sampling $S_1$ and $S_2$ also require $O(n)$ time. Computing a point in the deepest cell of $\Arr(\hat{S})$ requires $f(|\hat{S}|)=f(\frac{1}{\eps^2}\log |\RangeSet|)$.
Identifying the cell $p_{\indx}$ and computing the coefficient for the required $v_{\indx}$ variable takes $O(n)$ time. Each attempt of the MWU requires at most $\frac{1}{\eps^2}\log |\RangeSet|$ iterations. Since $\eps=\frac{\delta}{16}$, the overall running time is $O((\log\frac{1}{\delta}+\log\log \frac{1}{\delta})(n+f(\frac{1}{\delta^2}\log^{\frac{d}{2}} |\RangeSet|))\frac{1}{\delta^2}\log |\RangeSet|)$.

If $\RangeSet$ consists of a set of rectangles then the deepest cell of $\Arr(\hat{S})$ can be computed in
$\Tilde{O}(|\hat{S}|^{d/2})=\Tilde{O}(\frac{1}{\eps^d}\log^{\frac{d}{2}} |\RangeSet|)$ time using standard techniques \cite{oy-nubkm-91}. The overall running time is $\Tilde{O}((\log\frac{1}{\delta}+\log\log \frac{1}{\delta})(n+\frac{1}{\delta^d}\log^{\frac{d}{2}} |\RangeSet|)\frac{1}{\delta^2}\log |\RangeSet|)=\tilde{O}(\frac{n}{\delta^2}+\frac{1}{\delta^{d+2}})$.

% \section{Pseudocode Alg}

% \paragraph{Algorithm}
% Let $\alpha \in [0,1]$ be a guess for the optimal error. Let $\eps=\frac{\delta}{16}$.
% We discretize the range $[0,1]$ into a list of errors $E=\{\frac{\eps}{2}, (1+\eps)\frac{\eps}{2}, (1+\eps)^2\frac{\eps}{2},\ldots, 1\}$. We guess the optimal error $\alpha$ by running a binary search on $E$.
% The algorithm starts with $\alpha$ set to the middle value of $E$ and tries to  find a distribution $\Dist'$ such that $\Error(\Dist',\TrainingSet)\leq \alpha+\eps$ using MWU.
% If it fails, it resets $\alpha$ to a larger value of $E$ following the binary search. If it succeeds, it resets $\alpha$ to a smaller value of $E$ following the binary search. In the end of the binary search, for a particular $\alpha$ that the MWU last succeeded, we get $\Dist'$.

% \paragraph{MWU} The MWU algorithm runs for $\iter=O(?)$ iterations. In each iteration, it adds at most one new point to a set $\F$. Initially, $\F=\emptyset$. If it successfully completes $\iter$ iterations it returns $\F$ assigning each point a weight of $\frac{1}{\iter}$.

% \par Before the first iteration, it sets up an array $\W$ of size $2n+1$. Let us assume that $\W$ is indexed starting from $0$. It will be convinient to split $W$ into three subsets: $\{W[0]\}$, $\Pos=\{W[1],...,W[n]\}$ and $\Neg=\{W[n+1],...,W[2n]\}$. We use $\Pos[i]$ (resp. $\Neg[i]$) to refer to $\W[i]$ (resp. $\W[n+i]$).
% Initially, $\W[i]=1$ for all $i\in \{0,...,2n\}$.


% \par 
% In a particular iteration, performs the following steps:

% \begin{enumerate}
%     \item The algorithm determines a threshold $\tau=\thres(W,\TrainingSet)$. 

%     \item The algorithm generates a subset of $S_1\subseteq \RangeSet$ by sampling $\kappa=O(\frac{1}{\eps^2}\log |\RangeSet|)$ rectangles where each range $R_j$ is sampled with probability  $\frac{\Pos[j]}{\sum\limits_{i=1}^n \Pos[i]}$. Similarly, generate another subset $S_2\subseteq \RangeSet$ by sampling $\kappa$ ranges where each rectangle $R_j$ is sampled with probability  $\frac{\Neg[j]}{\sum\limits_{i=1}^n \Neg[i]}$. 

%     \item Let $\hat{S}=S_1\cup S_2$ be a weighted set of ranges where each range in $S_1$ has weight $\frac{w(\Pos)}{\kappa}$ and each range. The algorithm uses $\alg$ to compute the deepest point $p$ in $\hat{S}$.

%     \item If $\depth(p)<\tau$, the algorithm aborts the present guess, else it add $p$ to $\F$.

%     \item Finally, it updates the weights i.e. $\W=\reweight(\W,\TrainingSet,p)$
% \end{enumerate}

% We describe the procedures $\thres$ and $\reweight$ in the course of the analysis.


\begin{algorithm}[t]
\caption{{\sc DetectTriangle}$(p,\eps, \tau, \tau')$}
\label{alg:detect-general}

$C_{p} \gets D(p,\tau,\tau',\eps/2)$\;
Assume $C_{p} = \{C_{p,1}, C_{p,2}, \cdots, C_{p,k}\}$\;
\ForEach{$j \in [k]$}{
   $\Lambda_j^p = 
    \left\{q \in \C_{p,j}: I^-_q \le I_p^-, I_p^- + \tau' \le I^+_q < I_p^- +\tau \right\}$\;
    $\Psi_j^p = \left\{q \in C_{p,j}: I_q^-\leq I_p^-, I_q^+\geq I_p^-+ \tau \right\}$\;
    \lIf{$|\mathcal{C}_{p,j}| \ge 2$ and $|\Lambda_j^p|\geq 1$}{\Return \textbf{true}}
}
\ForEach{$(h,j) \in [k] \times [k]$ with $h \neq j$}{
        \If{$\phi(\textsf{rep}_h, \textsf{rep}_j) \le 1 + \frac{\epsilon}{2}$ and $|C_{p,h}|\ge 1$ and $|C_{p,j}| \ge 1$ and $|\Lambda_h^p\cup \Lambda_j^p|\geq 1$}{
            \Return \textbf{true}\;
        }
    
    }
\Return \textbf{false}\;
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newpage
% \subsection{Algorithm}
% Let $\alpha \in [0,1]$ be a guess for the optimal error. Let $\eps=\frac{\delta}{16}$.
% We discretize the range $[0,1]$ into a list of errors $E=\{\frac{\eps}{2}, (1+\eps)\frac{\eps}{2}, (1+\eps)^2\frac{\eps}{2},\ldots, 1\}$. We guess the optimal error $\alpha$ by running a binary search on $E$.
% The algorithm starts with $\alpha$ set to the middle value of $E$ and tries to  find a distribution $\Dist''$ such that $\Error(\Dist'',\TrainingSet)\leq \alpha+\eps$ using MWU.
% If it fails, it resets $\alpha$ to a larger value of $E$ following the binary search. If it succeeds, it resets $\alpha$ to a smaller value of $E$ following the binary search. In the end of the binary search, 
% for a particular $\alpha$ that the MWU last succeeded, we get $\Dist''$. The algorithm computes an $\eps$-approximation of $\Dist''$ and returns it as the output $\Dist'$.

% %If it fails, it resets $\alpha:=\max(1,(1+\eps)\alpha)$ and restarts. For a particular $\alpha$, if the MWU concludes and outputs $\Dist''$, the algorithm computes an $\eps$-approximation of $\Dist''$ and returns it as the output $\Dist'$.
% \par In a particular attempt at running MWU, the algorithm tries to iteratively solve the the following optimization problem:
% %\paragraph{LP 1}
% \begin{align*}
%  \\
%  \quad & \\
%  & \frac{1}{n}\sum_{R_i\in\RangeSet} z_i\leq \alpha \quad \\
% & z_i=|\sum_{p_j\in\P\cap R_i}v_j- s_i| \quad \forall R_i\in\RangeSet\\
% & v_j\geq 0 \quad \forall p_j\in \P\\
% & \sum_{p_j\in \P} v_j\leq 1 \\
% & z_i\in [0,1] \quad \forall R_i\in \RangeSet
% \end{align*}
% The fact that the above optimization problem does not require the sum of the weights to be 1 is not of concern since it is trivial to find a point that lies outside $\RangeSet$ and assign it the remaining mass. Consider the following equivalent LP: 
%  \paragraph{LP 2}
% \begin{align*}
%  \\
%  \quad & \\
%  & \sum_{R_i\in\RangeSet}-\frac{z_i}{n}\geq -\alpha \quad \text{(Type \RNum{1})} \\
% & z_i+\sum_{p_j\in\P\cap R_i}v_j\geq s_i \quad \forall R_i\in\RangeSet \quad \text{(Type \RNum{2})}\\
% &  z_i-\sum_{p_j\in\P\cap R_i}v_j\geq -s_i \quad \forall R_i\in\RangeSet \quad \text{(Type \RNum{3})}\\
% & \sum_{p_j\in \P} v_j\leq 1 \quad \text{(Type \RNum{4})}\\
% & v_j\geq 0 \quad \forall p_j\in \P \quad \text{(Type \RNum{4})}\\
% & z_i\in [0,1] \quad \forall R_i\in \RangeSet \quad \text{(Type \RNum{4})}
% \end{align*}
% In any attempt, the MWU runs for $T=O(\frac{\ln(|\RangeSet|)}{\eps^2})$ iterations. Let $\F$ be a multi-set that is empty initially. In each iteration, the MWU process adds at most one point to $\F$. At the end of $T$ rounds, it returns the discrete distribution with support $\F$ where each point has weight $\frac{1}{T}$.\footnote{Note that the sum of weights of all points may be less than 1.}   Let $\MA\vx\geq \vb$ be the matrix-vector representation of the LP 2 ignoring the Type \RNum{4} constraints. Thus, $\MA$ is the constraint matrix, $\vx$ is the vector representing the variables, and $\vb$ is a vector representing the RHS of the constraints. The MWU algorithm maintains a probability vector $\vp$ whose dimension equals the number of rows of $\MA$. Thus $dim(\vp)=2|\RangeSet|+1$.
% Let us denote the coordinate in $\vp$ with respect to the $j$-th Type \RNum{2} (resp. Type \RNum{3}) constraint by $\vpos_j$ (resp. $\vpneg_j$).
% Let $Pos$ (resp. $Neg$) be the collection of coordinates of vector $\vp$ with respect to  Type \RNum{2} (resp. Type \RNum{3}) constraints.
% %  Let $Pos$ (resp. $Neg$) be the collection of coordinates of the form $\vpos_j$ (resp. $\vpneg_j$).
% Note that $|Pos|=|Neg|=|\RangeSet|$. Let $w(Pos)=\sum_{j\in Pos}\vpos_j$ (resp. $w(Neg)=\sum_{j\in Neg}\vpneg_j$) denote the sum of all values in $Pos$ (resp. $Neg$). Initially $\vp$ represents the uniform distribution. In each iteration $t$, the MWU algorithm checks if there exists a solution $\vx^{(t)}$ satisfying all Type \RNum{4} constraints such that $\vp^T\MA\vx^{(t)}\geq \vp^T\vb-\frac{\eps}{2}$ holds.

% \paragraph{Checking Feasibility} Consider the expansion of the expression $\vp^T\MA\vx$. Observe that the LHS is of the form $\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{1}{n}C^{-}_i)z_{i}+\sum\limits_{p_j\in\P}(D^{+}_j-D^{-}_j)v_j$ where $C_i^{+}$ and $ D_j^{+}$ (resp. $C_i^{-}$ and $ D_j^{-}$) represent the sum of all positive (resp. negative) coefficients of each $z_i$ and $v_j$ in the expansion of $\vp^T\MA\vx$ respectively.

% For any $i\leq |\RangeSet|$, we compute $C_i^+=\vpos_{i}+\vpneg_{i}$. Furthermore, $C_i^-=\vp_1$.
% There is no non-trivial type \RNum{4} constraint for variables $z_i$, so for each $z_i^{(t)}$, set $z_i^{(t)}:=0$, if $(C^{+}_i-\frac{1}{n}C^{-}_i)\leq 0$, else set $z_i^{(t)}:=1$. Finally, we set $\gamma_1=\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{1}{n}C^{-}_i)z_{i}^{(t)}$. 


% Next, we focus on setting the variables $v_j$, which is a more challenging task because the are $O(n^d)$ of them and there are non-trivial Type \RNum{4} constraints. 
% We use an $\eps$-approximation schema to set the variables $v_j$ by (approximately) maximizing $\vp^T\MA\vx$.
% We generate a subset of $S_1\subseteq \RangeSet$ by sampling $\kappa=O(\frac{1}{\eps^2}\log |\RangeSet|)$ rectangles where each rectangle $R_j$ is sampled with probability  $\frac{\vpos_j}{w(Pos)}$. Similarly, generate another subset $S_2\subseteq \RangeSet$ by sampling $\kappa$ rectangles where each rectangle $R_j$ is sampled with probability  $\frac{\vpneg_j}{w(Neg)}$. Let $\hat{S}=S_1\cup S_2$ be a weighted set of rectangles where each rectangle in $S_1$ has weight $\frac{w(Pos)}{\kappa}$ and each rectangle in $S_2$ has weight $-\frac{w(Neg)}{\kappa}$. Let $\square$ be the cell in $\Arr(\hat{S})$, the arrangement of $\hat{S}$, of maximum weighted depth. Take an arbitrary point $l_{\square}$ in $\square$.
% \newcommand{\indx}{j^{l_\square}}
% We find all rectangles in $\RangeSet$ that contain $l_\square$, so we can identify the index $\indx$ such that $p_{\indx}\in \P$ is contained in the same set of rectangles in $\RangeSet$ as the point $l_\square$.
% We compute $D^{+}_{\indx}=\sum_{i: p_{\indx}\in R_i}\vpos_{i}$ and $D^{-}_{\indx}=\sum_{i: p_{\indx}\in R_i}\vpneg_{i}$.


% If $\gamma+\max(0, (D^{+}_{\indx}-D^{-}_{\indx}))+\frac{\eps}{2}<\vp^T\vb$, declare that the current $\alpha$ is too small and abort the MWU. On the other hand, if $\gamma+max(0,(D^{+}_{\indx}-D^{-}_{\indx}))+\frac{\eps}{2}\geq \vp^T\vb$, then  if $D^{+}_{\indx}-D^{-}_{\indx}>0$, add $l_{\square}$ to $\F$.
% %Let $v_{\indx}$ be the variable in LP 2 corresponding to the point $l_{\square}$.
% If $(D^{+}_{\indx}-D^{-}_{\indx})>0$, consider $x^{(t)}$ to be the solution determined by setting each $z_i^{(t)}$ as above and ${v_{\indx}^{(t)}=1}$. Else, consider $x^{(t)}$ to be the solution determined by setting each $z_i^{(t)}$ as above and all $v_{\indx}^{(t)}=0$.

% Next, the MWU requires to update each coordinate $\vp_j$ of $\vp$ such that ${\vp_j}^{(t+1)}:={\vp_j}^{(t)}\frac{(1-\eta (\MA_j\vx_j^{(t)}-b_j))}{\Phi^{(t)}} $. Depending on the constraint corresponding to $A_i$, the expression $(\MA_j\vx_j-b_j)$ can be determined from the computed values of each $z_i^{(t)}$ in the current iteration as well as checking if the rectangle corresponding to $\vp_j$ contains the point $l_{\square}$. Here $\eta=\frac{\eps}{12}$ and $\Phi^{(t)}$ is a normalizing constant to ensure $\vp$ remains a distribution. After updating $\vp$, the algorithm then moves on to the next iteration.



% % Assign an integer label to each constraint in the above LP except for the last two constraints. The MWU algorithm maintains a non-negative weight $\beta_j$ for each constraint with label $j$. Note that there are $2|\RangeSet|+1$ such constraints. In the first iteration, $\forall j$,$B_j:=1$. In a particular iteration, the algorithm checks if the weighted sum of the contraints, where co 



% \subsection{Analysis}
% \paragraph{Correctness}  Suppose LP 2 has a feasible solution. Observe that for $\forall i\quad |\MA_i\vx-b_i|\in [-2,2]$. Therefore, by Theorem 3.5 of [AroraMWU], if in each iteration of the MWU, the algorithm can find a solution $\vx^{(t)}$ satisfying all Type \RNum{4} constraints such that $\vp^T\MA\vx^{(t)}\geq \vp^T\vb-\frac{\eps}{2}$ holds then after $T=O(\frac{\ln(|\RangeSet|)}{\eps^2})$ iterations, it is true that $\forall i\quad \MA_i\vx\geq \vb_i-\eps$ holds where $\vx=\frac{1}{T}\sum\limits_{t=1}^T \vx^{(t)}$. Assuming the algorithm checks feasibility in each iteration successfully, the description of the algorithm suggests that  $\vx=\frac{1}{T}\sum\limits_{t=1}^T \vx^{(t)}$ is equivalent to the discrete distribution with support $\F$ where each point has weight $\frac{1}{T}$. Because each $z_i$ may not capture the error of $R_i$ exactly, this implies $\Error(\Dist_{\F},\TrainingSet)\leq \Error(OPT,\TrainingSet)+3\eps$. Now it remains to prove that the algorithm can check feasibility in each iteration accurately. 

% \par Observe that checking if there exists an $\vx$ such that $\vp^T\MA\vx \geq \vp^T\vb-\frac{\varepsilon}{2}$ under Type $\RNum{4}$ constraints is equivalent to maximizing $\vp^T\MA\vx$ under Type $\RNum{4}$ constraints. Recall that, $\vp^T\MA\vx=\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{1}{n}C^{-}_i)z_{i}+\sum\limits_{p_j\in\P}(D^{+}_j-D^{-}_j)v_j$. Furthermore, note that the two summations can be maximized independently because they do not have common variables. It is easy to verify that the algorithm maximizes $\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{1}{n}C^{-}_i)z_{i}$.
% For the term $\sum\limits_{p_j\in\P}(D^{+}_j-D^{+}_j)v_j$, observe that this is maximized by setting the variable with the largest coefficient to one if it is non-negative or else setting everything to zero. This is because $\sum\limits_{p_j\in \P} v_j\leq 1$. Let $v_{j^*}$ denote the variable with the largest coefficient. Recall $v_{\indx}$ is the variable found by the algorithm through the sampling step. 
% \begin{lemma}
% $(D^{+}_{\indx}-D^{-}_{\indx})\geq (D^{+}_{j^{*}}-D^{-}_{j^*})-\eps $
% \end{lemma}
% \begin{proof}
% Consider the range space $\Sigma=(\Re^d,S_1)$ and its dual $\Sigma^D$. Since $|S_1|=\kappa=O(\frac{1}{\eps^2}\log |\RangeSet|)$, it is known that $S_1$ is an $\frac{\eps}{4}$-approximation for $\Sigma^D$ with probability at least $1-n^{O(d)}$. More specifically, it holds that  $|\frac{w_1(p_{j^*})}{\kappa}- \frac{D^{+}_{j^{*}}}{w(Pos)}|\leq \frac{\eps}{4}$, where $w_1(p_{j^*})$ denotes the  number of rectangles in $S_1$ containing $p_{j^*}$. Similarly, $S_2$ is is an $\frac{\eps}{4}$-approximation for $\Sigma^D$, so it holds that $|\frac{w_2(p_{j^*})}{\kappa}- \frac{D^{-}_{j^{*}}}{w(Neg)}|\leq \frac{\eps}{4}$, where $w_2(p_{j^*})$ denotes the  number of rectangles in $S_2$ containing $p_{j^*}$.
% Equivalently, using the fact that $w(Pos)\in [0,1]$ and $w(Neg)\in [0,1]$, we can rewrite the inequalities above as,
% $$D_{j^*}^+-\frac{\eps}{4}\leq w_1(p_{j^*})\frac{w(Pos)}{\kappa}\leq D_{j^*}^++\frac{\eps}{4}$$
% $$D_{j^*}^--\frac{\eps}{4}\leq w_2(p_{j^*})\frac{w(Neg)}{\kappa}\leq D_{j^*}^-+\frac{\eps}{4},$$
% so it follows that,
% $$D_{j^*}^+-D_{j^*}^--\frac{\eps}{2}\leq w_1(p_{j^*})\frac{w(Pos)}{\kappa}-w_2(p_{j^*})\frac{w(Neg)}{\kappa}\leq D_{j^*}^+-D_{j^*}^-+\frac{\eps}{2}.$$
% The same inequalities hold for any point in $\Re^d$, for example $l_\square$.
% Recall that the algorithm chooses a point $l_\square$ in the cell $\square$ of $\Arr(\hat{S})$ with the maximum weighted depth.
% By the inequalities above, it holds that,
% $$D^{+}_{\indx}-D^{-}_{\indx}\geq w_1(l_\square)\frac{w(Pos)}{\kappa}-w_2(l_\square)\frac{w(Neg)}{\kappa}-\frac{\eps}{2}\geq w_1(p_{j^*})\frac{w(Pos)}{\kappa}-w_2(p_{j^*})\frac{w(Neg)}{\kappa}-\frac{\eps}{2}\geq D_{j^*}^+-D_{j^*}^--\eps.$$


% %Together, they imply that for any point lying in a particular cell $\Delta$ of $\Arr(\hat{S}=S_1\cup S_2)$  (where each rectangle in $S_1$ has weight $\frac{w(Pos)}{\kappa}$ and each rectangle in $S_2$ has weight $-\frac{w(Neg)}{\kappa}$) the coefficient of its corresponding variable in $\vp^T\MA\vx$ is within $\frac{\eps}{4}$ of the weight of $\Delta$ in $\Arr(\hat{S})$. In particular this implies $v_{\indx}$ has coefficient at least $D^{+}_{j^{*}}-D^{-}_{j^{*}}-\frac{\eps}{2}$. 

% \end{proof}

% In any iteration of the MWU for $\alpha\geq \Error(OPT,\TrainingSet)$
% %$\alpha\in [\max(\frac{\eps}{2}, \Error(OPT,\TrainingSet)),\max(\frac{\eps}{2}, (1+\eps)\Error(OPT,\TrainingSet))]$,
% there exists a feasible solution, and therefore $max(0,D^{+}_{j^{*}}-D^{-}_{j^{*}})\geq\vp^T\vb-\gamma $. The above lemma implies $max(0,D^{+}_{j^{*}}-D^{-}_{j^{*}})-\max(0, (D^{+}_{\indx}-D^{-}_{\indx}) )\leq \frac{\eps}{2}$. Therefore, $\gamma+\max(0, w(l_{\square}))+\frac{\eps}{2}\geq \vp^T\vb$ must hold. This concludes the proof that the algorithm always finds a feasible solution when $\alpha$ in the above range.
% \par Combining above along with the fact that the algorithm take an $\eps$-approximation (recall $\eps=\frac{\delta}{16}$)  at the end implies, $|\Dist'|\leq O(\frac{1}{\delta^2}\log\frac{1}{\delta})$ and $\Error(\Dist',\TrainingSet)\leq \Error(OPT,\TrainingSet)+\delta$ with high probability. 
% \paragraph{Running Time}
% The size of $E$ is $O(\frac{1}{\eps}\log\frac{1}{\eps})$ so the algorithm requires $O(\log\frac{1}{\eps}+\log\log\frac{1}{\eps})$ attempts.
% %Since the algorithm starts with $\alpha=\frac{\eps}{2}$ and increases $\alpha$ by a factor of $(1+\eps)$ in each new attempt, it requires $O(\frac{1}{\eps}\log \frac{1}{\eps})$ attempts.
% In each iteration of MWU, the coefficients of all the $z_i$ along with $\gamma$ can be computed in $O(n)$ time. Sampling $S_1$ and $S_2$ also require $O(n)$ time. Computing a point in the deepest cell of $\Arr(\hat{S})$ requires $f(|hat{S}|)=f(\frac{1}{\eps^2}\log |\RangeSet|)$.
% Identifying the cell $p_{\indx}$ and computing the coefficient for the required $v_{\indx}$ variable takes $O(n)$ time. Each attempt of the MWU requires at most $\frac{1}{\eps^2}\log |\RangeSet|$ iterations. Since $\eps=\frac{\delta}{16}$, the overall running time is $O((\log\frac{1}{\delta}+\log\log \frac{1}{\delta})(n+f(\frac{1}{\delta^2}\log^{\frac{d}{2}} |\RangeSet|))\frac{1}{\delta^2}\log |\RangeSet|)$.

% If $\RangeSet$ consists of a set of rectangles then the deepest cell of $\Arr(\hat{S})$ can be computed in
% $\Tilde{O}(|\hat{S}|^{d/2})=\Tilde{O}(\frac{1}{\eps^d}\log^{\frac{d}{2}} |\RangeSet|)$ time using standard techniques \cite{oy-nubkm-91}. The overall running time is $\Tilde{O}((\log\frac{1}{\delta}+\log\log \frac{1}{\delta})(n+\frac{1}{\delta^d}\log^{\frac{d}{2}} |\RangeSet|)\frac{1}{\delta^2}\log |\RangeSet|)=\tilde{O}(\frac{n}{\delta^2}+\frac{1}{\delta^{d+2}})$.

==> Misc/fromRIP.tex <==
\section{New}

Consider the range space $\Sigma=(\GroundSet,\RangeSet)$  where $\GroundSet=\Re^d$ and $\RangeSet$ is a collection of boxes. Let $\TrainingSet=\{z_1,...,z_n\}$ be a set of boxes along with their associated weights, i.e., $z_i=(R_i,s_i)\in \RangeSet\times[0,1]$. A \emph{discrete distribution} $\Dist$ is defined by a finite set of points and their corresponding weights, $\Dist=\{(p_1,w_1),...,(p_m,w_m)\}$, where each $p_i$ is a point in $\Re^d$, and $\sum_{i=1}^m w_i\leq 1$. In this section, we describe an algorithm for computing a small sized discrete distribution such that the sum of weights of points placed inside each box in $\TrainingSet$ is close to its associated weight (on average). The parallels between computing a discrete distribution  and piercing are self-evident.
  The piercing problem essentially asks for the discrete distribution with fewest points such that each box has positive weight.
  
  
  
  
  
  % For a query range $R\in R$, $s_{\Dist}(R):=\sum_{i=1}^m \mathbf{1}(p_i\in R)w_i$.

\paragraph{Background} Let $\Sigma=(\GroundSet,\RangeSet)$ be a range space. Let $\Dist$ denote a probability distribution over $\GroundSet$. Then, the selectivity of a range $R\in \RangeSet$ with respect to $\Dist$, denoted $s_{\Dist}(R)$, is defined as $s_{\Dist}(R):=\Pr_{x\sim \Dist}[x\in R]$. 
For a range space $\Sigma=(\GroundSet,\RangeSet)$,
a subset $P\subseteq \GroundSet$ is shattered by $\RangeSet$ if $\{P\cap \RangeSet\mid R\in \RangeSet\}=2^P$. The VC-dimension of $\RangeSet$, denoted by \textit{VC-dim}$(\Sigma)$, is the size of the largest subset of $\GroundSet$ that can be shattered by $\Sigma$. Let $\DistFam$ denote a set of distributions defined on $\GroundSet$. Let $S_{\Sigma,\DistFam}=\{s_D\mid \Dist\in\DistFam \}$, be a family of selectivity functions from $\RangeSet$ to $[0,1]$.  Using classic learning theory for real-valued functions, \cite{sel1} show that if the \textit{VC-dim}$(\Sigma)=\lambda$, where $\lambda$ is some constant, then the family of selectivity functions $S_{\Sigma,\mathbb{D}}$ is $\eps$-\textit{learnable} using $\Tilde{O}(\frac{1}{\eps^{\lambda+3}})$ samples\footnote{See Theorem 2.1 of \cite{sel1} for exact details.}. The definition of $\eps$-\textit{learnable} assumes the existence of an algorithm which given a set of training samples  $\TrainingSet=\{z_1,...,z_n\}$ where each $z_i=(R_i,s_i)\in \RangeSet\times[0,1]$ and a family of distributions $\mathbb{D}$, finds a $\Dist\in\mathbb{D}$
that minimizes the expected loss function\footnote{ The framework in \cite{sel1} can also be extended to other error functions such as $L_1$ and $L_{\infty}$.}  i.e. $\min_{\Dist\in\DistFam}\frac{1}{n}\sum_{i=1}^n(s_{\Dist}(R_i)-s_i)^2$ or $\min_{\Dist\in\DistFam}\frac{1}{n}\sum_{i=1}^n|s_{\Dist}(R_i)-s_i|$. For picking $\DistFam$, the family of data distributions, discrete distributions are a natural choice. 


\paragraph{Related work}
There exists a rich body of work on estimating selectivity of range queries. Historically, database systems have attempted to estimate selectivity by computing some kind of a synopsis of the joint distribution of attributes. Recent works have focused more on machine learning based techniques.  \par Early works treated the data as input and learned the underlying data distribution via histograms. Histograms group the data into buckets and maintain the summary statistics of each bucket. In \cite{DBLP:conf/vldb/JagadishKMPSS98}, the authors used dynamic programming to compute optimal histograms for one-dimensional data. For higher dimensions, \cite{DBLP:conf/sigmod/MuralikrishnaD88}, \cite{DBLP:conf/vldb/PoosalaI97}, \cite{DBLP:conf/sigmod/PoosalaIHS96} designed efficient heuristics but did not offer any theoretical guarantees on the performance. In \cite{DBLP:conf/icdt/MuthukrishnanPS99}, the authors showed that for most natural metrics, computing multi-dimensional histograms is NP-hard even in 2-dimensions. Another set of works also also used histograms to summarise the data distribution but only using past queries as input \cite{DBLP:conf/sigmod/BrunoCG01}, \cite{DBLP:conf/icde/SrivastavaHMKT06}, \cite{DBLP:conf/sigmod/ParkZM20}. 
\par Machine learning based techniques are more often hybrid, they use both the data and prior queries. The learning is mostly based on prior queries while the data is used for enriching the training queries and validation. \cite{DBLP:conf/cidr/KipfKRLBK19}, \cite{DBLP:journals/pvldb/DuttWNKNC19}, \cite{DBLP:conf/sigmod/HasanTAK020} present models based on neural networks for orthogonal range queries. \cite{DBLP:conf/sigmod/WangXQ0SWO20} and \cite{DBLP:conf/sigmod/Sun0021} use deep learning based techniques for distance based queries.
\par The most relevant work to our project is by \cite{sel1}. Using classic learning theory for real-valued functions they show that selectivity can be learned from a small number of samples for a large class of range queries. The learning itself requires building a model of the underlying data distribution based on sample queries. They describe a generic algorithm with theoretically guaranteed performance that works for histograms and discrete distributions. Their procedure requires computing the arrangement of the ranges. This makes the running time $\Omega(n^d)$ which becomes infeasible as $d$ grows. In order to overcome this dependence, they focus on histograms and discrete distributions with a bounded number of buckets. They note that based on hardness results for related problems, this restriction is likely to make the problem NP-hard (which turns out to be true at least for discrete distributions). They design efficient heuristics that perform well in practice but do not offer any theoretical guarantees on the performance.
% \par While not directly related to selectivity estimation, the Geometric Hitting Set problem has some resemblance to the problem of computing the optimal discrete distribution using the minimum number of buckets. 
 % Let $\Sigma=(X,R)$ be a range space. A subset $H\subseteq R$ is called a hitting set if it intersects every range in $R$. In the geometric variant, objects are typically a set of points and ranges are geometric regions. We are particularly interested in the cases where the ranges are axis-parallel rectangles, balls and half-spaces. For $d=2$, \cite{DBLP:journals/dcg/AgarwalP20} give a near linear time approximation with an approximation ratio of $O(\log\log OPT)$ for rectangles, and $O(1)$ for half-spaces and disks. For d=3, \cite{DBLP:conf/compgeom/MustafaR09} give a PTAS when the ranges are half-spaces. However, \cite{DBLP:journals/comgeo/ChanG14} show that the problem is APX-hard for axis-parallel rectangles for $d=2$, balls for $d=3$, and half-spaces for $d=4$.



 \paragraph{Our Result} In this section, we build on the work of \cite{sel1}. We design a fast algorithm that finds a small discrete distribution with performance guarantees. For a discrete distribution $\Dist$ and a training set $\TrainingSet$ let the error of $\Dist$ on $\TrainingSet$ be defined as $\Error(\Dist, \TrainingSet)=\frac{1}{n}\sum_{i=1}^n|(s_{\Dist}(R_i)-s_i)|$.   Let $OPT=arg\min_{\Dist\in\DistFam}\Error(\Dist, \TrainingSet)$. We prove the following: 
 
 % Let $f(|\RangeSet|)$ be a function for the time it takes to compute the weighted deepest point in the arrangement $\Arr(\RangeSet)$. Our main result, proved in Section 3, is the following:   
 
\begin{theorem}
There exists an algorithm that takes as input a set of training samples,\\ $\TrainingSet=\{(R_1,s_1),\dots, (R_n,s_n)\}$    
where each $R_i$ is a box in $\mathbb{R}^d$ and $s_i\in [0,1]$ is its corresponding selectivity, and a parameter $\delta\in (0,1)$, and returns a discrete distribution $\Dist'$ of size $|\Dist'|=O(d\frac{1}{\delta^2}\log\frac{1}{\delta})$ such that $\Error(\Dist',\TrainingSet)\leq \Error(OPT,\TrainingSet)+\delta$ with high probability. Furthermore, the algorithm takes $O((\log\frac{1}{\delta}+\log\log \frac{1}{\delta})(n+\frac{1}{\delta^d}\log^{\frac{d}{2}} n)\frac{1}{\delta^2}\log n)=\tilde{O}(\frac{n}{\delta^2}+\frac{1}{\delta^{d+2}})$ time.  \end{theorem}


% \begin{corollary}
% If $\RangeSet$ comprises of rectangles, the above algorithm takes time
% \begin{equation*}
%     O(\frac{1}{\delta}\log \frac{1}{\delta}(n+(\frac{1}{\delta^2}\log |\RangeSet|)^{\frac{d}{2}})\frac{1}{\delta^2}\log |\RangeSet|)=\tilde{O}(\frac{n}{\delta^3}+\frac{1}{\delta^{d+3}})
% \end{equation*}

% \end{corollary}



%$\mathcal{E}(\mathscr{Z})$. 


\begin{remark}
    The above algorithm can be easily modified to handle $L_{2}$ and $L_{\infty}$ errors with the same performance guarantees.
\end{remark}


\subsection{MWU Algorithm}

\paragraph{Plan} Let $\P=\{p_1,...,p_m\}$  be a finite subset of $\Re^d$ such that it contains exactly one point from each cell in $\Arr(\RangeSet)$. Consider the following optimization problem on $|\P|$ variables where each variable $v_i$ corresponds to the point $p_i\in \P$.

\begin{align*}
\text{minimize} \quad & \frac{1}{n}\sum_{i=1}^n|(\sum_{p_j\in\P\cap R_i}v_j- s_i)| \\
\text{subject to} \quad & \\
& \sum_{p_j\in \P} v_j= 1 \\
& v_j\geq 0 \quad \forall p_j\in \P
\end{align*}

It is easy to see that an optimal solution to the above LP gives an optimal discrete distribution in terms of error. However, computing this can be very expensive as the arrangement may have $\Theta(n^d)$ cells. Our strategy is to solve this optimization problem using the MWU as described in \cite{v008a006} without explicitly constructing all the variables. We note that a straightforward implementation of the MWU method in our problem  also leads to $\Omega(n^d)$ time due to the number of variables. Hence, new ideas are needed to overcome this obstacle.




\paragraph{Algorithm}
Let $\alpha \in [0,1]$ be a guess for the optimal error. Let $\eps=\frac{\delta}{16}$.
We discretize the range $[0,1]$ into a list of errors $E=\{\frac{\eps}{2}, (1+\eps)\frac{\eps}{2}, (1+\eps)^2\frac{\eps}{2},\ldots, 1\}$. We guess the optimal error $\alpha$ by running a binary search on $E$.
The algorithm starts with $\alpha$ set to the middle value of $E$ and tries to  find a distribution $\Dist''$ such that $\Error(\Dist'',\TrainingSet)\leq \alpha+\eps$ using MWU.
If it fails, it resets $\alpha$ to a larger value of $E$ following the binary search. If it succeeds, it resets $\alpha$ to a smaller value of $E$ following the binary search. In the end of the binary search, 
for a particular $\alpha$ that the MWU last succeeded, we get $\Dist''$. The algorithm computes an $\eps$-approximation of $\Dist''$ and returns it as the output $\Dist'$.

%If it fails, it resets $\alpha:=\max(1,(1+\eps)\alpha)$ and restarts. For a particular $\alpha$, if the MWU concludes and outputs $\Dist''$, the algorithm computes an $\eps$-approximation of $\Dist''$ and returns it as the output $\Dist'$.
\par In a particular attempt at running MWU, the algorithm tries to iteratively solve the the following optimization problem:
%\paragraph{LP 1}
\begin{align*}
 \\
 \quad & \\
 & \frac{1}{n}\sum_{R_i\in\RangeSet} z_i\leq \alpha \quad \\
& z_i=|\sum_{p_j\in\P\cap R_i}v_j- s_i| \quad \forall R_i\in\RangeSet\\
& v_j\geq 0 \quad \forall p_j\in \P\\
& \sum_{p_j\in \P} v_j\leq 1 \\
& z_i\in [0,1] \quad \forall R_i\in \RangeSet
\end{align*}
The fact that the above optimization problem does not require the sum of the weights to be 1 is not of concern since it is trivial to find a point that lies outside $\RangeSet$ and assign it the remaining mass. Consider the following equivalent LP: 
 \paragraph{LP 2}
\begin{align*}
 \\
 \quad & \\
 & \sum_{R_i\in\RangeSet}-\frac{z_i}{n}\geq -\alpha \quad \text{(Type \RNum{1})} \\
& z_i+\sum_{p_j\in\P\cap R_i}v_j\geq s_i \quad \forall R_i\in\RangeSet \quad \text{(Type \RNum{2})}\\
&  z_i-\sum_{p_j\in\P\cap R_i}v_j\geq -s_i \quad \forall R_i\in\RangeSet \quad \text{(Type \RNum{3})}\\
& \sum_{p_j\in \P} v_j\leq 1 \quad \text{(Type \RNum{4})}\\
& v_j\geq 0 \quad \forall p_j\in \P \quad \text{(Type \RNum{4})}\\
& z_i\in [0,1] \quad \forall R_i\in \RangeSet \quad \text{(Type \RNum{4})}
\end{align*}
In any attempt, the MWU runs for $T=O(\frac{\ln(|\RangeSet|)}{\eps^2})$ iterations. Let $\F$ be a multi-set that is empty initially. In each iteration, the MWU process adds at most one point to $\F$. At the end of $T$ rounds, it returns the discrete distribution with support $\F$ where each point has weight $\frac{1}{T}$.\footnote{Note that the sum of weights of all points may be less than 1.}   Let $\MA\vx\geq \vb$ be the matrix-vector representation of the LP 2 ignoring the Type \RNum{4} constraints. Thus, $\MA$ is the constraint matrix, $\vx$ is the vector representing the variables, and $\vb$ is a vector representing the RHS of the constraints. The MWU algorithm maintains a probability vector $\vp$ whose dimension equals the number of rows of $\MA$. Thus $dim(\vp)=2|\RangeSet|+1$.
Let us denote the coordinate in $\vp$ with respect to the $j$-th Type \RNum{2} (resp. Type \RNum{3}) constraint by $\vpos_j$ (resp. $\vpneg_j$).
Let $Pos$ (resp. $Neg$) be the collection of coordinates of vector $\vp$ with respect to  Type \RNum{2} (resp. Type \RNum{3}) constraints.
%  Let $Pos$ (resp. $Neg$) be the collection of coordinates of the form $\vpos_j$ (resp. $\vpneg_j$).
Note that $|Pos|=|Neg|=|\RangeSet|$. Let $w(Pos)=\sum_{j\in Pos}\vpos_j$ (resp. $w(Neg)=\sum_{j\in Neg}\vpneg_j$) denote the sum of all values in $Pos$ (resp. $Neg$). Initially $\vp$ represents the uniform distribution. In each iteration $t$, the MWU algorithm checks if there exists a solution $\vx^{(t)}$ satisfying all Type \RNum{4} constraints such that $\vp^T\MA\vx^{(t)}\geq \vp^T\vb-\frac{\eps}{2}$ holds.

\paragraph{Checking Feasibility} Consider the expansion of the expression $\vp^T\MA\vx$. Observe that the LHS is of the form $\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{1}{n}C^{-}_i)z_{i}+\sum\limits_{p_j\in\P}(D^{+}_j-D^{-}_j)v_j$ where $C_i^{+}$ and $ D_j^{+}$ (resp. $C_i^{-}$ and $ D_j^{-}$) represent the sum of all positive (resp. negative) coefficients of each $z_i$ and $v_j$ in the expansion of $\vp^T\MA\vx$ respectively.

For any $i\leq |\RangeSet|$, we compute $C_i^+=\vpos_{i}+\vpneg_{i}$. Furthermore, $C_i^-=\vp_1$.
There is no non-trivial type \RNum{4} constraint for variables $z_i$, so for each $z_i^{(t)}$, set $z_i^{(t)}:=0$, if $(C^{+}_i-\frac{1}{n}C^{-}_i)\leq 0$, else set $z_i^{(t)}:=1$. Finally, we set $\gamma_1=\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{1}{n}C^{-}_i)z_{i}^{(t)}$. 


Next, we focus on setting the variables $v_j$, which is a more challenging task because the are $O(n^d)$ of them and there are non-trivial Type \RNum{4} constraints. 
We use an $\eps$-approximation schema to set the variables $v_j$ by (approximately) maximizing $\vp^T\MA\vx$.
We generate a subset of $S_1\subseteq \RangeSet$ by sampling $\kappa=O(\frac{1}{\eps^2}\log |\RangeSet|)$ rectangles where each rectangle $R_j$ is sampled with probability  $\frac{\vpos_j}{w(Pos)}$. Similarly, generate another subset $S_2\subseteq \RangeSet$ by sampling $\kappa$ rectangles where each rectangle $R_j$ is sampled with probability  $\frac{\vpneg_j}{w(Neg)}$. Let $\hat{S}=S_1\cup S_2$ be a weighted set of rectangles where each rectangle in $S_1$ has weight $\frac{w(Pos)}{\kappa}$ and each rectangle in $S_2$ has weight $-\frac{w(Neg)}{\kappa}$. Let $\square$ be the cell in $\Arr(\hat{S})$, the arrangement of $\hat{S}$, of maximum weighted depth. Take an arbitrary point $l_{\square}$ in $\square$.
\newcommand{\indx}{j^{l_\square}}
We find all rectangles in $\RangeSet$ that contain $l_\square$, so we can identify the index $\indx$ such that $p_{\indx}\in \P$ is contained in the same set of rectangles in $\RangeSet$ as the point $l_\square$.
We compute $D^{+}_{\indx}=\sum_{i: p_{\indx}\in R_i}\vpos_{i}$ and $D^{-}_{\indx}=\sum_{i: p_{\indx}\in R_i}\vpneg_{i}$.


If $\gamma+\max(0, (D^{+}_{\indx}-D^{-}_{\indx}))+\frac{\eps}{2}<\vp^T\vb$, declare that the current $\alpha$ is too small and abort the MWU. On the other hand, if $\gamma+max(0,(D^{+}_{\indx}-D^{-}_{\indx}))+\frac{\eps}{2}\geq \vp^T\vb$, then  if $D^{+}_{\indx}-D^{-}_{\indx}>0$, add $l_{\square}$ to $\F$.
%Let $v_{\indx}$ be the variable in LP 2 corresponding to the point $l_{\square}$.
If $(D^{+}_{\indx}-D^{-}_{\indx})>0$, consider $x^{(t)}$ to be the solution determined by setting each $z_i^{(t)}$ as above and ${v_{\indx}^{(t)}=1}$. Else, consider $x^{(t)}$ to be the solution determined by setting each $z_i^{(t)}$ as above and all $v_{\indx}^{(t)}=0$.

Next, the MWU requires to update each coordinate $\vp_j$ of $\vp$ such that ${\vp_j}^{(t+1)}:={\vp_j}^{(t)}\frac{(1-\eta (\MA_j\vx_j^{(t)}-b_j))}{\Phi^{(t)}} $. Depending on the constraint corresponding to $A_i$, the expression $(\MA_j\vx_j-b_j)$ can be determined from the computed values of each $z_i^{(t)}$ in the current iteration as well as checking if the rectangle corresponding to $\vp_j$ contains the point $l_{\square}$. Here $\eta=\frac{\eps}{12}$ and $\Phi^{(t)}$ is a normalizing constant to ensure $\vp$ remains a distribution. After updating $\vp$, the algorithm then moves on to the next iteration.



% Assign an integer label to each constraint in the above LP except for the last two constraints. The MWU algorithm maintains a non-negative weight $\beta_j$ for each constraint with label $j$. Note that there are $2|\RangeSet|+1$ such constraints. In the first iteration, $\forall j$,$B_j:=1$. In a particular iteration, the algorithm checks if the weighted sum of the contraints, where co    
\subsection{Analysis}
\paragraph{Correctness}  Suppose LP 2 has a feasible solution. Observe that for $\forall i\quad |\MA_i\vx-b_i|\in [-2,2]$. Therefore, by Theorem 3.5 of [AroraMWU], if in each iteration of the MWU, the algorithm can find a solution $\vx^{(t)}$ satisfying all Type \RNum{4} constraints such that $\vp^T\MA\vx^{(t)}\geq \vp^T\vb-\frac{\eps}{2}$ holds then after $T=O(\frac{\ln(|\RangeSet|)}{\eps^2})$ iterations, it is true that $\forall i\quad \MA_i\vx\geq \vb_i-\eps$ holds where $\vx=\frac{1}{T}\sum\limits_{t=1}^T \vx^{(t)}$. Assuming the algorithm checks feasibility in each iteration successfully, the description of the algorithm suggests that  $\vx=\frac{1}{T}\sum\limits_{t=1}^T \vx^{(t)}$ is equivalent to the discrete distribution with support $\F$ where each point has weight $\frac{1}{T}$. Because each $z_i$ may not capture the error of $R_i$ exactly, this implies $\Error(\Dist_{\F},\TrainingSet)\leq \Error(OPT,\TrainingSet)+3\eps$. Now it remains to prove that the algorithm can check feasibility in each iteration accurately. 

\par Observe that checking if there exists an $\vx$ such that $\vp^T\MA\vx \geq \vp^T\vb-\frac{\varepsilon}{2}$ under Type $\RNum{4}$ constraints is equivalent to maximizing $\vp^T\MA\vx$ under Type $\RNum{4}$ constraints. Recall that, $\vp^T\MA\vx=\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{1}{n}C^{-}_i)z_{i}+\sum\limits_{p_j\in\P}(D^{+}_j-D^{-}_j)v_j$. Furthermore, note that the two summations can be maximized independently because they do not have common variables. It is easy to verify that the algorithm maximizes $\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{1}{n}C^{-}_i)z_{i}$.
For the term $\sum\limits_{p_j\in\P}(D^{+}_j-D^{+}_j)v_j$, observe that this is maximized by setting the variable with the largest coefficient to one if it is non-negative or else setting everything to zero. This is because $\sum\limits_{p_j\in \P} v_j\leq 1$. Let $v_{j^*}$ denote the variable with the largest coefficient. Recall $v_{\indx}$ is the variable found by the algorithm through the sampling step. 
\begin{lemma}
$(D^{+}_{\indx}-D^{-}_{\indx})\geq (D^{+}_{j^{*}}-D^{-}_{j^*})-\eps $
\end{lemma}
\begin{proof}
Consider the range space $\Sigma=(\Re^d,S_1)$ and its dual $\Sigma^D$. Since $|S_1|=\kappa=O(\frac{1}{\eps^2}\log |\RangeSet|)$, it is known that $S_1$ is an $\frac{\eps}{4}$-approximation for $\Sigma^D$ with probability at least $1-n^{O(d)}$. More specifically, it holds that  $|\frac{w_1(p_{j^*})}{\kappa}- \frac{D^{+}_{j^{*}}}{w(Pos)}|\leq \frac{\eps}{4}$, where $w_1(p_{j^*})$ denotes the  number of rectangles in $S_1$ containing $p_{j^*}$. Similarly, $S_2$ is is an $\frac{\eps}{4}$-approximation for $\Sigma^D$, so it holds that $|\frac{w_2(p_{j^*})}{\kappa}- \frac{D^{-}_{j^{*}}}{w(Neg)}|\leq \frac{\eps}{4}$, where $w_2(p_{j^*})$ denotes the  number of rectangles in $S_2$ containing $p_{j^*}$.
Equivalently, using the fact that $w(Pos)\in [0,1]$ and $w(Neg)\in [0,1]$, we can rewrite the inequalities above as,
$$D_{j^*}^+-\frac{\eps}{4}\leq w_1(p_{j^*})\frac{w(Pos)}{\kappa}\leq D_{j^*}^++\frac{\eps}{4}$$
$$D_{j^*}^--\frac{\eps}{4}\leq w_2(p_{j^*})\frac{w(Neg)}{\kappa}\leq D_{j^*}^-+\frac{\eps}{4},$$
so it follows that,
$$D_{j^*}^+-D_{j^*}^--\frac{\eps}{2}\leq w_1(p_{j^*})\frac{w(Pos)}{\kappa}-w_2(p_{j^*})\frac{w(Neg)}{\kappa}\leq D_{j^*}^+-D_{j^*}^-+\frac{\eps}{2}.$$
The same inequalities hold for any point in $\Re^d$, for example $l_\square$.
Recall that the algorithm chooses a point $l_\square$ in the cell $\square$ of $\Arr(\hat{S})$ with the maximum weighted depth.
By the inequalities above, it holds that,
$$D^{+}_{\indx}-D^{-}_{\indx}\geq w_1(l_\square)\frac{w(Pos)}{\kappa}-w_2(l_\square)\frac{w(Neg)}{\kappa}-\frac{\eps}{2}\geq w_1(p_{j^*})\frac{w(Pos)}{\kappa}-w_2(p_{j^*})\frac{w(Neg)}{\kappa}-\frac{\eps}{2}\geq D_{j^*}^+-D_{j^*}^--\eps.$$


%Together, they imply that for any point lying in a particular cell $\Delta$ of $\Arr(\hat{S}=S_1\cup S_2)$  (where each rectangle in $S_1$ has weight $\frac{w(Pos)}{\kappa}$ and each rectangle in $S_2$ has weight $-\frac{w(Neg)}{\kappa}$) the coefficient of its corresponding variable in $\vp^T\MA\vx$ is within $\frac{\eps}{4}$ of the weight of $\Delta$ in $\Arr(\hat{S})$. In particular this implies $v_{\indx}$ has coefficient at least $D^{+}_{j^{*}}-D^{-}_{j^{*}}-\frac{\eps}{2}$. 
\end{proof}

In any iteration of the MWU when $\alpha\in [\max(\frac{\eps}{2}, \Error(OPT,\TrainingSet)),\max(\frac{\eps}{2}, (1+\eps)\Error(OPT,\TrainingSet))]$, a feasible solution exists, and therefore $max(0,D^{+}_{j^{*}}-D^{-}_{j^{*}})\geq\vp^T\vb-\gamma $. The above lemma implies $max(0,D^{+}_{j^{*}}-D^{-}_{j^{*}})-\max(0, (D^{+}_{\indx}-D^{-}_{\indx}) )\leq \frac{\eps}{2}$. Therefore, $\gamma+\max(0, w(l_{\square}))+\frac{\eps}{2}\geq \vp^T\vb$ must hold. This concludes the proof that the algorithm always finds a feasible solution when $\alpha$ in the above range.
\par Combining above along with the fact that the algorithm take an $\eps$-approximation (recall $\eps=\frac{\delta}{16}$)  at the end implies, $|\Dist'|\leq O(\frac{1}{\delta^2}\log\frac{1}{\delta})$ and $\Error(\Dist',\TrainingSet)\leq \Error(OPT,\TrainingSet)+\delta$ with high probability. 
\paragraph{Running Time}
The size of $E$ is $O(\frac{1}{\eps}\log\frac{1}{\eps})$ so the algorithm requires $O(\log\frac{1}{\eps}+\log\log\frac{1}{\eps})$ attempts.
%Since the algorithm starts with $\alpha=\frac{\eps}{2}$ and increases $\alpha$ by a factor of $(1+\eps)$ in each new attempt, it requires $O(\frac{1}{\eps}\log \frac{1}{\eps})$ attempts.
In each iteration of MWU, the coefficients of all the $z_i$ along with $\gamma$ can be computed in $O(n)$ time. Sampling $S_1$ and $S_2$ also require $O(n)$ time. Computing a point in the deepest cell of $\Arr(\hat{S})$ requires $\Tilde{O}(|\hat{S}|^{d/2})=\Tilde{O}(\frac{1}{\eps^d}\log^{\frac{d}{2}} |\RangeSet|)$ time using standard techniques \cite{oy-nubkm-91}. Identifying the cell $p_{\indx}$ and computing the coefficient for the required $v_{\indx}$ variable takes $O(n)$ time. Each attempt of the MWU requires at most $\frac{1}{\eps^2}\log |\RangeSet|$ iterations. Since $\eps=\frac{\delta}{16}$, the overall running time is $O((\log\frac{1}{\delta}+\log\log \frac{1}{\delta})(n+(\frac{1}{\delta^d}\log^{\frac{d}{2}} |\RangeSet|))\frac{1}{\delta^2}\log |\RangeSet|)=\tilde{O}(\frac{n}{\delta^2}+\frac{1}{\delta^{d+2}})$. 

==> Misc/prefix_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
%%% Comment out to use biblatex instead of bibtex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
% \def\UseBibLatex{1}

\newif\ifSoCG
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%% Comment out to get regular version
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%% \SoCGtrue


\makeatletter
\def\input@path{{styles/}{../styles/}}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ifSoCG
    \newcommand{\SoCGVer}[1]{#1}
    \newcommand{\RegVer}[1]{}
\else
    \newcommand{\SoCGVer}[1]{}
    \newcommand{\RegVer}[1]{#1}
\fi

%\RegVer{
%    \documentclass[12pt]{article}
%    \usepackage[cm]{fullpage}
%    \usepackage{euscript}
%}
 
%\SoCGVer{
%\documentclass[a4paper,UKenglish,cleveref, autoref, thm-restate,anonymous]{socg-lipics-v2021}
%}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{amsfonts} \usepackage{xcolor} \usepackage{graphicx}
\usepackage{xspace}%
\usepackage{hyperref}%
%\usepackage{upgreek}%
%\usepackage{wsuipa}%

   %ocgcolorlinks,
\hypersetup{%
   breaklinks,%
   colorlinks=true,%
   urlcolor=[rgb]{0.25,0.0,0.0},%
   linkcolor=[rgb]{0.5,0.0,0.0},%
      citecolor=[rgb]{0,0.2,0.445},%
      filecolor=[rgb]{0,0,0.4},
      anchorcolor=[rgb]={0.0,0.1,0.2}%
   }
   

\usepackage{algorithm}
\usepackage[noend]{algpseudocode}

   % \def\reals{\mathbb{R}}
\newcommand{\eps}{\varepsilon}%

\let\bd\partial
\def\ph{\varphi}


\let\Horig\H
 
%\def\A{\mathcal{A}\fogi}%
%\def\B{\mathcal{B}\fogi}%
%\def\D{\mathcal{D}\fogi}%
%\def\E{\mathcal{E}\fogi}%
%\def\EP{\mathcal{E}\fogi}%
\def\C{\mathcal{C}}%
\def\F{\mathcal{F}}%
\def\FS{\mathcal{F}}%
\def\J{\mathcal{J}}%
\def\K{\mathcal{K}}
\def\L{\mathcal{L}}
%\def\N{\mathcal{N}}
%\def\P{\mathcal{P}}
\def\R{\mathcal{R}\flogi}
\def\T{\mathcal{T}}
\def\H{\mathcal{H}}
%\def\N{\mathcal{N}}
\def\W{\mathcal{W}}
\def\O{\widetilde{O}}
 %%%%%%%%%%%%%
 %%%%%%%%%%%%%
\def\ES{\mathbb{E}}
\def\QQ{\mathcal{Q}}
%%%%%%%%%%%%%
%\def\V{\mathcal{V}}

%%%%%%% Macros for operations
\newcommand{\weight}{\AlgorithmI{weight}\xspace}%
\newcommand{\update}{\AlgorithmI{update}\xspace}%
\newcommand{\sample}{\AlgorithmI{sample}\xspace}%
\newcommand{\query} {\AlgorithmI{query}\xspace}%
%%%%%%%
% These macros are to include in-line comments.
\def\marrow{\marginpar[\hfill$\longrightarrow$]{$\longleftarrow$}}
\def\pankaj#1{\textcolor{red}{\textsc{(Pankaj says: }\marrow\textsf{#1})}}
\def\rahul#1{\textsc{(Rahul says: }\marrow\textsf{#1})}
%% The following is supposed to swallow comments, DO NOT use in production, as it might have weird spacing effects.

%\long\def\newtext#1{{\color{red} #1}}

%\def\mparagraph#1{\par\medskip\noindent{\textbf{#1.}}\quad\parindent 1.5em}

%\renewcommand{\widetilde}{1]{#1}


\long\def\newtext#1{ #1}

\usepackage{amsmath}%
\usepackage{amssymb}%


\RegVer{%
   \usepackage[amsmath,thmmarks]{ntheorem}%
   \theoremseparator{.}%
   
   \usepackage{titlesec}%
   \titlelabel{\thetitle. }%
   
   % ----------------------------------------------------------------------
   % ----------------------------------------------------------------------
   % Defining theorem like environments
   % ----------------------------------------------------------------------
   % ----------------------------------------------------------------------
   \theoremseparator{.}%
   
   \theoremstyle{plain}%
   \newtheorem{theorem}{Theorem}[section]
   
   \newtheorem{lemma}[theorem]{Lemma}
   \newtheorem{conjecture}[theorem]{Conjecture}
   \newtheorem{corollary}[theorem]{Corollary}
   \newtheorem{claim}[theorem]{Claim}%
   \newtheorem{fact}[theorem]{Fact}
   \newtheorem{observation}[theorem]{Observation}
   \newtheorem{invariant}[theorem]{Invariant}
   \newtheorem{question}[theorem]{Question}
   \newtheorem{proposition}[theorem]{Proposition}
   \newtheorem{prop}[theorem]{Proposition}
   \newtheorem{openproblem}[theorem]{Open Problem}
   
   \theoremstyle{plain}%
   \theoremheaderfont{\sf} \theorembodyfont{\upshape}%
   \newtheorem*{remark:unnumbered}[theorem]{Remark}%
   \newtheorem*{remarks}[theorem]{Remarks}%
   \newtheorem{remark}[theorem]{Remark}%
   \newtheorem{definition}[theorem]{Definition}
   \newtheorem{defn}[theorem]{Definition}
   \newtheorem{example}[theorem]{Example}
   \newtheorem{exercise}[theorem]{Exercise}
   \newtheorem{problem}[theorem]{Problem}
   \newtheorem{xca}[theorem]{Exercise}
   \newtheorem{exercise_h}[theorem]{Exercise}
   \newtheorem{assumption}[theorem]{Assumption}%
   
   % Proof environment
   \newcommand{\myqedsymbol}{\rule{2mm}{2mm}}
   
   \theoremheaderfont{\em}%
   \theorembodyfont{\upshape}%
   \theoremstyle{nonumberplain}%
   \theoremseparator{}%
   \theoremsymbol{\myqedsymbol}%
   \newtheorem{proof}{Proof:}%
   
   \newtheorem{proofof}{Proof of\!}%
   
   % theorem block end
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
}
\RegVer{%
   \numberwithin{figure}{section}%
   \numberwithin{table}{section}%
   \numberwithin{equation}{section}%
}%

\usepackage{mleftright}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 5
% Color emph
\providecommand{\emphind}[1]{\emph{#1}\index{#1}}
\definecolor{blue25emph}{rgb}{0, 0, 11}
\providecommand{\emphic}[2]{%
   \textcolor{blue25emph}{%
      \textbf{\emph{#1}}}%
   \index{#2}}

\providecommand{\emphi}[1]{\emphic{#1}{#1}}

\definecolor{almostblack}{rgb}{0, 0, 0.3}
\providecommand{\emphw}[1]{{\textcolor{almostblack}{\emph{#1}}}}%

\providecommand{\emphOnly}[1]{\emph{\textcolor{blue25}{\textbf{#1}}}}
% Color emph - end 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 5




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% thank you, thank you!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

\providecommand{\tildegen}{{\protect\raisebox{-0.1cm}
      {\symbol{'176}\hspace{-0.01cm}}}}
\newcommand{\atgen}{\symbol{'100}} \newcommand{\SarielThanks}[1]{%
   \thanks{%
      Department of Computer Science; University of Illinois; 201
      N. Goodwin Avenue; Urbana, IL, 61801, USA; {\tt
         sariel\atgen{}illinois.edu};
      {\tt \url{http://sarielhp.org/}.} #1
   }%
}

\newcommand{\PankajThanks}[1]{%
   \thanks{%
      Department of Computer Science, Duke University, Durham NC
      27708. %
      #1
   }%
}
\newcommand{\RahulThanks}[1]{%
   \thanks{%
      Department of Computer Science, Duke University, Durham NC
      27708. %
      #1
   }%
}
\newcommand{\StavrosThanks}[1]{%
   \thanks{%
        Department of Computer Science. University of Illinois at Chicago, Chicago IL 60607. %
      #1
   }%
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    Handling references
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\HLink}[2]{\hyperref[#2]{#1~\ref*{#2}}}
\newcommand{\HLinkSuffix}[3]{\hyperref[#2]{#1\ref*{#2}{#3}}}

\newcommand{\figlab}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{\HLink{Figure}{fig:#1}}

\newcommand{\thmlab}[1]{{\label{theo:#1}}}
\newcommand{\thmref}[1]{\HLink{Theorem}{theo:#1}}

\newcommand{\corlab}[1]{\label{cor:#1}}
\newcommand{\corref}[1]{\HLink{Corollary}{cor:#1}}%

\newcommand{\apndlab}[1]{\label{apnd:#1}}
\newcommand{\apndref}[1]{\HLink{Appendix}{apnd:#1}}

\newcommand{\seclab}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{\HLink{Section}{sec:#1}}


\newcommand{\itemlab}[1]{\label{item:#1}}
\newcommand{\itemref}[1]{\HLinkSuffix{}{item:#1}{}}
\newcommand{\itemrefY}[2]{\hyperref[item:#2]{#1}}

\providecommand{\deflab}[1]{\label{def:#1}}
\newcommand{\defref}[1]{\HLink{Definition}{def:#1}}

\newcommand{\lemlab}[1]{\label{lemma:#1}}
\newcommand{\lemref}[1]{\HLink{Lemma}{lemma:#1}}%

\providecommand{\eqlab}[1]{}%
\renewcommand{\eqlab}[1]{\label{equation:#1}}
\newcommand{\Eqref}[1]{\HLinkSuffix{Eq.~(}{equation:#1}{)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% Sariel's standard commands...
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

\newcommand{\remove}[1]{}%
\newcommand{\Set}[2]{\left\{ #1 \;\middle\vert\; #2 \right\}}
\newcommand{\pth}[2][\!]{\mleft({#2}\mright)}%
\newcommand{\pbrcx}[1]{\left[ {#1} \right]}%
\newcommand{\Prob}[1]{\mathop{\mathbf{Pr}}\!\pbrcx{#1}}
\newcommand{\Ex}[2][\!]{\mathop{\mathbf{E}}#1\pbrcx{#2}}

\newcommand{\ceil}[1]{\left\lceil {#1} \right\rceil}
\newcommand{\floor}[1]{\left\lfloor {#1} \right\rfloor}

\newcommand{\brc}[1]{\left\{ {#1} \right\}}
\newcommand{\cardin}[1]{\left| {#1} \right|}%

\renewcommand{\th}{th\xspace}
\newcommand{\ds}{\displaystyle}%

\newcommand{\ZZ}{\mathbb{Z}}%
\renewcommand{\Re}{\mathbb{R}}%
\newcommand{\reals}{\Re}%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Defining comptenum environment using enumitem
\usepackage[inline]{enumitem}

\newlist{compactenumA}{enumerate}{5}%
\setlist[compactenumA]{topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex,%
   label=(\Alph*)}%

\newlist{compactenuma}{enumerate}{5}%
\setlist[compactenuma]{topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex,%
   label=(\alph*)}%

\newlist{compactenumI}{enumerate}{5}%
\setlist[compactenumI]{topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex,%
   label=(\Roman*)}%

\newlist{compactenumi}{enumerate}{5}%
\setlist[compactenumi]{topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex,%
   label=(\roman*)}%

\newlist{compactitem}{itemize}{5}%
\setlist[compactitem]{topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex,%
   label=\ensuremath{\bullet}}%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Biblatex....
%
\providecommand{\BibLatexMode}[1]{}
\providecommand{\BibTexMode}[1]{#1}

\ifx\UseBibLatex\undefined%
  \renewcommand{\BibLatexMode}[1]{}
  \renewcommand{\BibTexMode}[1]{#1}
\else
  \renewcommand{\BibLatexMode}[1]{#1}
  \renewcommand{\BibTexMode}[1]{}
\fi


% Bib latex stuff
\BibLatexMode{%
   \dsdfaa
   \usepackage[bibencoding=utf8,style=alphabetic,backend=biber]{biblatex}%
   \usepackage{sariel_biblatex}%
}

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% Papers specific commands...
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\providecommand{\Mh}[1]{#1}%

\newcommand{\IS}{\Mh{\mathsf{IS}}}%
%\newcommand{\ISX}[1]{\IS\pth{#1}}
\newcommand{\ISX}[1]{\mathcalb{I}\pth{#1}} %substitution
%\newcommand{\fIS}{\Mh{\mathsf{f}_\mathsf{IS}}}
\newcommand{\fIS}{\mathcalb{I}^*} %substitution
\newcommand{\PN}{\Mh{\mathsf{PN}}}%
%\newcommand{\PNX}[1]{\PN\pth{#1}}
\newcommand{\PNX}[1]{\mathbcalb{k}\pth{#1}} %substitution
%\newcommand{\fPN}{\Mh{\mathsf{f}_\mathsf{PN}}}
\newcommand{\fPN}{\mathbcalb{k}^{*}} 
\newcommand{\Dist}{\mathcal{D}} %substitution

\newcommand{\AlgPierce}{\AlgorithmI{Pierce}\xspace}%
\newcommand{\TPierce}{\ensuremath{T_\AlgorithmI{P}\xspace}}%
\newcommand{\Partition}{\Mh{\Pi}}
\newcommand{\Term}[1]{\textsf{#1}}
\newcommand{\TermI}[1]{\Term{#1}\index{#1@\Term{#1}}}

\newcommand{\LP}{\Term{LP}\xspace}%
\newcommand{\MWU}{\Term{MWU}\xspace}
\newcommand{\ts}{\hspace{0.6pt}}

\newcommand{\Face}{\Mh{\mathsf{f}}}%
\newcommand{\rstY}[2]{#1_{| #2}}%
\newcommand{\nrstY}[2]{\Mh{\#}\pth{#2, #1}}%
\newcommand{\nInY}[2]{\Mh{\#}\pth{#1, #2}}
\newcommand{\wY}[2]{\wC\pth{#1, #2}}
\newcommand{\depthX}[1]{\mathrm{depth}\pth{#1}}%

\renewcommand{\S}{\Mh{\mathcal{S}}}%
\newcommand{\U}{\Mh{\mathcal{U}}}%
\newcommand{\I}{\Mh{\EuScript{I}}}

\newcommand{\projY}[2]{#1_{\downarrow #2}}%
\newcommand{\XX}{\Mh{\mathcal{X}}}
\newcommand{\YY}{\Mh{\mathcal{Y}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%BeginIpePreamble
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \newcommand{\eps}{\Mh{\varepsilon}}

%%%%%%%%%

\newcommand{\Eps}{\Mh{\mathcal{E}}}
%\newcommand{\eps}{\Mh{\varepsilon}}
\newcommand{\epsA}{\Mh{\vartheta}}

%%%%%%%%


%\newcommand{\epsA}{\Mh{\vartheta}}

\newcommand{\si}[1]{#1}
\newcommand{\N}{\Mh{\mathcal{N}}}
% \newcommand{\X}{\Mh{\mathcal{X}}}
% \newcommand{\G}{\Mh{\mathcal{G}}}

\newcommand{\X}{\Mh{\mathcal{X}}}
\newcommand{\Q}{\Mh{\mathcal{Q}}}
\renewcommand{\P}{\Mh{\mathcal{P}}}


\RegVer{%
   % Add period after paragraph title...
   \titleformat{\paragraph}[runin]
   {\normalfont\bfseries}
   {\theparagraph}
   {1em}
   {\addperiod}

   \newcommand{\addperiod}[1]{#1.}

   \titlespacing{\paragraph}{0pt}{2ex}{0.2cm}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \mathcalb - a different font that looks a bit like mathcal

\DeclareFontFamily{U}{BOONDOX-calo}{\skewchar\font=45 }
\DeclareFontShape{U}{BOONDOX-calo}{m}{n}{
  <-> s*[1.05] BOONDOX-r-calo}{}
\DeclareFontShape{U}{BOONDOX-calo}{b}{n}{
  <-> s*[1.05] BOONDOX-b-calo}{}
\DeclareMathAlphabet{\mathcalb}{U}{BOONDOX-calo}{m}{n}
\SetMathAlphabet{\mathcalb}{bold}{U}{BOONDOX-calo}{b}{n}
\DeclareMathAlphabet{\mathbcalb}{U}{BOONDOX-calo}{b}{n}

% \mathcalb - end of file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\providecommand{\TPDF}[2]{\texorpdfstring{#1}{#2}}
\newcommand{\hrefb}[3][black]{\href{#2}{\color{#1}{#3}}}%

\newcommand{\Dim}{\Mh{d}}%
\newcommand{\BadProb}{\Mh{\varphi}}%
\newcommand{\DistFam}{\mathbb{D}}
\newcommand{\TrainingSet}{\mathcal{Z}}
\newcommand{\GroundSet}{\mathcal{X}}
\newcommand{\GroundSetB}{\textsf{Y}}
\newcommand{\FGroundSet}{\mathsf{X}}

\newcommand{\Error}{\mathcal{E}}
\newcommand{\Family}{\Mh{\mathcal{F}}}%
\newcommand{\SetC}{\Mh{C}}%
%\newcommand{\range}{\Mh{\mathbf{r}}}
\newcommand{\range}{\Mh{\mathsf{R}}} % substitution
\newcommand{\MeasureChar}{\overline{m}}
\newcommand{\sMeasureChar}{\overline{s}}
\newcommand{\Measure}[1]{\MeasureChar\pth{#1}}
\newcommand{\MeasureX}[2]{\MeasureChar_{#2}\pth{#1}}
\newcommand{\sMeasure}[1]{\overline{s}\pth{#1}}
\newcommand{\sMeasureX}[2]{\overline{s}_{#2}\pth{#1}}
\newcommand{\sMeasureXC}[1]{\overline{s}_{#1}}

\newcommand{\Grid}{\Mh{\EuScript{G}}}%
\newcommand{\Arr}{\Mh{\mathop{\mathrm{\EuScript{A}}}}}
\newcommand{\ArrX}[1]{\Arr\pth{#1}}%


\newcommand{\etal}{\textit{et~al.}\xspace}

\newcommand{\Edges}{\mathsf{E}}%
\providecommand{\Bronnimann}{Br{\"o}nnimann\xspace}

\newcommand{\opt}{\Mh{OPT}}
\newcommand{\alg}{DEEPEST}
\newcommand{\depth}{depth}
\newcommand{\Pos}{\W^+}
\newcommand{\Neg}{{\W}^{-}}
\newcommand{\iter}{\mathcal{T}}
\newcommand{\thres}{Threshold}
\newcommand{\val}{Val}
\newcommand{\reweight}{Reweight}



\DefineNamedColor{named}{AlgorithmColor}{cmyk}{0.07,0.90,0,0.34}

\newcommand{\AlgorithmI}[1]{{%
      \textcolor[named]{AlgorithmColor}{\texttt{\bf{#1}}}%
   }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% from prefix 2
\newcommand{\ii}{\mathcalb{i}}

\usepackage{stmaryrd}%
\providecommand{\IntRange}[1]{\mleft\llbracket #1 \mright\rrbracket}
\newcommand{\IRX}[1]{\IntRange{#1}}%
\newcommand{\IRY}[2]{\left\llbracket #1:#2 \right\rrbracket}
\newcommand{\nQ}{\Mh{\mathcalb{n}}}%
\newcommand{\nG}{\Mh{n_\Grid}}%
% \newcommand{\R}{\Mh{\mathcal{R}}}%


\newcommand{\RangeSet}{{\Mh{\mathcal{R}}}}

\newcommand{\RangeSpace} {\Mh{\mathsf{S}}}

%\newcommand{\rect}{\Mh{\mathsf{r}}}%
\newcommand{\rect}{\mathcal{R}}% substitution
%\newcommand{\bb}{\Mh{\mathsf{b}}}% 
\newcommand{\bb}{\Mh{\mathsf{B}}}% substitution
\newcommand{\bbA}{\Mh{\mathsf{c}}}%
\newcommand{\bbB}{\Mh{\mathsf{d}}}%

%\newcommand{\cell}{\Mh{\mathsf{c}}}%
\newcommand{\cell}{\Mh{\mathsf{\tau}}}% substitution

\newcommand{\Sample}{\Mh{\mathcal{S}}}%
\newcommand{\Boxes}{\Mh{\mathcal{B}}}%
\newcommand{\ListB}{\Mh{\mathcal{S}}}%
\newcommand{\LightB}{\Mh{\mathcal{L}}}%
\newcommand{\HeavyB}{\Mh{\mathcal{H}}}%
\newcommand{\IndepB}{\Mh{\mathcal{I}}}%
\newcommand{\Crates}{\Mh{\mathcal{T}}}%
\newcommand{\Cells}{\Mh{\mathcal{C}}}%
\newcommand{\LCells}{\Mh{\mathcal{L}}}%
\newcommand{\shrinkX}[1]{\mathrm{shrink}\pth{#1}}%
\newcommand{\lgEps}{\Mh{\ell}}%
\newcommand{\nMass}{\Mh{\mathcalb{w}}}%

\newcommand{\dst}{\Mh{\mathcal{D}}}%

\newcommand{\Line}{\Mh{\mathcalb{l}}}%
\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}
\newcommand{\nRounds}{\Mh{\zeta}}%

\newcommand{\polylog}{\mathop{\mathrm{polylog}}}%
\newcommand{\VV}{\Mh{\mathcal{V}}}%
\newcommand{\VX}[1]{\VV\pth{#1}}

\newcommand{\wC}{\Mh{\omega}}
\newcommand{\wX}[1]{\wC\pth{#1}}%
\newcommand{\awX}[1]{\wC_\approx\pth{#1}}%

\newcommand{\hwC}{\Mh{\mathcalb{w}}}
\newcommand{\hwX}[1]{\hwC\pth{#1}}
%\newcommand{\hwY}[2]{\hwC\pth{#1, #2}}
\newcommand{\hwY}[2]{\hwC^{}_{\!#2}\pth{#1}}

 \newcommand{\vb}{ \mathbf{b}}
\newcommand{\vx}{ \mathbf{x}}
\newcommand{\vp}{ \mathbf{p}}
\newcommand{\vpos}{ \hat{\mathbf{p}}}
\newcommand{\vpneg}{ \bar{\mathbf{p}}}
\newcommand{\MA}{ \mathbf{A}}%
\newcommand{\mm}{\mathcalb{m}\!\ts}%

\newcommand{\ISet}{\Mh{\mathcal{I}}}%
%\newcommand{\Tree}{\Mh{\mathcal{T}}}%
\newcommand{\Tree}{\Mh{\mathfrak{T}}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%EndIpePreamble
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
% Conditional compilation depending on whether this is my computer or
% not.
\IfFileExists{sariel_computer.sty}{\def\sarielComp{1}}{}
\ifx\sarielComp\undefined%
\else
\usepackage{sariel_colors}%
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 





==> backup/basic_backup.tex <==
\section{Basic Algorithm}
\par Let $\TrainingSet=\{z_1,...,z_n\}$ be a set of training samples such that $z_i=(R_i,s_i)$ where $R_i$ is a range in $\Re^d$ and $s_i\in[0,1]$ is its selectivity. Let $\RangeSet:=\{R_1,...,R_n\}$ denote the set of ranges in $\TrainingSet$. Recall that for a discrete distribution $\Dist\in\mathbb{D}$,
\begin{equation*}
\Error(\Dist, \TrainingSet) =  \frac{1}{n}\sum_{i=1}^n \cardin{{s_{\Dist}(R_i) - s_i}}
\end{equation*}

Let $\opt:= \min_{\Dist\in\DistFam} \Error(\Dist, \TrainingSet)$. In this section, we design an algorithm that finds a discrete distribution $\Dist$ of size $\cardin{\Dist}\leq O(\frac{1}{\delta^2}\log n)$ such that $\Error(\Dist,\TrainingSet)\leq \opt+\delta$ where $\delta\in [0,1]$ is a given parameter.

\par For now, let us ignore the size condition and focus on finding a discrete distribution $\Dist$ that only satisfies the error condition i.e. $\Error(\Dist,\TrainingSet)\leq \opt+\delta$. Moreover, let us assume that we know the value of $\opt$. Our task then reduces to solving the following \emph{feasibility problem}:
\paragraph{\textbf{FP 1}}
\label{FP:1}
\begin{align*} 
%\quad & \\
 & \frac{1}{n}\sum_{R_i\in\RangeSet} u_i\leq \opt+\delta \quad \quad  \\
& u_i\geq |s_D(R_i)-s_i| \quad \forall\, R_i\in\RangeSet \quad \\
& u_i\in [0,1] \quad \forall\,R_i\in\RangeSet\\
& \Dist\in \DistFam
\end{align*}

Given that $\DistFam$ comprises of all discrete distributions, the solution space for the above appears to be infinite. However, it turns out that we can always restrict ourselves to a finite class.

\par The \emph{arrangement} of $\RangeSet$ denoted $\Arr(\RangeSet)$ is a partition of $\Re^d$ into contiguous regions called \emph{cells} such that each cell lies in the same subset of $\RangeSet$. Let $\P\subset \Re^d$ be the smallest set of points such that $\forall\, \square\in\Arr(\RangeSet)$, $\,|\P\cap\square|=1$ i.e. $\P$ contains exactly one point from every cell $\square$ of $\Arr(\RangeSet)$.
\begin{lemma} \lemlab{restrict}
    For any discrete distribution $\Dist$, there is another discrete distribution $\Dist'$ such that the support of $\Dist'$ is a subset of $\P$ and $\Error(\Dist,\TrainingSet)=\Error(\Dist',\TrainingSet)$.
\begin{proof}
First, observe that WLOG we can assume that the support of $\Dist$ does not contain any point that lies outside every range in $\RangeSet$. This is because such a point has no influence on $\Error(\Dist,\TrainingSet)$. Consider a point $q$ in the support of $\Dist$ that lies inside some $R_i\in \RangeSet$. There must exist some cell $\square\in \Arr(\RangeSet)$ such that 
$\square\cap q\neq \emptyset$. Let $p_i$ be the point in $\P$ corresponding to $\square$. Consider the distribution $\hat{\Dist}$ obtained by removing $q$ and adding its mass to $p_i$. Observe that $\Error(\Dist,\TrainingSet)=\Error(\hat{\Dist},\TrainingSet)$. This is because $p_i$ and $q$ are both contained by exactly the same subset of ranges of $\RangeSet$. By performing the previous steps  for finitely many repetitions we can obtain a distribution $\Dist'$ whose support is a subset of $\P$ and $\Error(\Dist,\TrainingSet)=\Error(\Dist',\TrainingSet)$.
\end{proof}
\end{lemma}
It is well known that $|\Arr(\RangeSet)|\leq O(n^d)$. Hence, $|\P|=O(n^d)$. Moreover, $\Arr(\RangeSet)$ ( and therefore $\P$) can be computed in $O(n^d\log n)$ time. Consider the following linear problem with variables $u_i$ for each range $R_i\in \RangeSet$ and $v_j$ for each point $p_j\in\P$.
\paragraph{\textbf{LP 1}} \label{LP:1}
\begin{align*}
 %\quad & \\
 & \frac{1}{n}\sum_{R_i\in\RangeSet} u_i\leq \opt+\delta \quad \\
& u_i=\cardin{\sum_{p_j\in\P\cap R_i}v_j- s_i} \quad \forall R_i\in\RangeSet\\
& v_j\geq 0 \quad \forall p_j\in \P\\
& \sum_{p_j\in \P} v_j\leq 1 \\
& u_i\in [0,1] \quad \forall R_i\in \RangeSet
\end{align*}
Let $\Dist_{\opt}$ be the discrete distribution with error $\opt$. By \lemref{restrict}, we can assume that support of $D_{\opt}$ is a subset of $\P$. Let $D_{\opt}$ assign weight $w_j$ to point $p_j\in \P$. By setting each $v_j:=w_j$ and each $u_i$ to the error of $R_i$ with respect to $D_{\opt}$, we obtain a feasible solution to the above LP. Similarly, it is easy to verify that a feasible solution to the above LP corresponds to valid discrete distribution with error $\opt+\delta$. 
\par We will now describe how to solve LP using the MWU method. Before proceeding, it will be useful for us to convert it into a canonical form.
\paragraph{\textbf{LP 2}}
\begin{align*}
 \\
 \quad & \\
 &\frac{1}{n} \sum_{R_i\in\RangeSet}-u_i\geq -\opt-\delta \quad \text{(Type \RNum{1})} \\
& u_i+\sum_{p_j\in\P\cap R_i}v_j\geq s_i \quad \forall R_i\in\RangeSet \quad \text{(Type \RNum{2})}\\
&  u_i-\sum_{p_j\in\P\cap R_i}v_j\geq -s_i \quad \forall R_i\in\RangeSet \quad \text{(Type \RNum{3})}\\
& \sum_{p_j\in \P} v_j\leq 1 \quad \text{(Type \RNum{4})}\\
& u_j\geq 0 \quad \forall p_j\in \P \quad \text{(Type \RNum{4})}\\
& u_i\in [0,1] \quad \forall R_i\in \RangeSet \quad \text{(Type \RNum{4})}
\end{align*}
\subsection{Using MWU to solve LP}
We now describe how to use MWU to solve the LP. Let $\MA\vx\geq \vb$ be the matrix-vector representation of the LP ignoring the Type \RNum{4} constraints. Thus, $\MA$ is the constraint matrix, $\vx$ is the vector representing the variables, and $\vb$ is a vector representing the RHS of the constraints. The MWU algorithm maintains a weight vector $\vp$ whose dimension equals the number of rows of $\MA$. Thus $dim(\vp)=2|\RangeSet|+1$. Let $\vone$ be the coordinate of in $\vp$ with respect to the only Type \RNum{1} constraint. Let the coordinate in $\vp$ with respect to the $j$-th Type \RNum{2} (resp. Type \RNum{3}) constraint by $\vpos_j$ (resp. $\vpneg_j$).
\par Let $\vp=\vp^{(0)}$ be the all ones vector initially. The MWU algorithm runs for $T=O(\frac{\ln(|\RangeSet|)}{\eps^2})$ iterations.  Let $\C$ be the set solutions to the LP satisfying all Type \RNum{4} constraints. In iteration $t$, MWU performs the following steps:

\begin{enumerate}
    \item Compute  $\vx^{(t)}=\arg\max_{\vx\in\C}\vp^T\MA\vx$. 
    
    \item If $\vp^T\MA\vx^{(t)}<\vp^T\vb+\frac{\delta}{2}$ abort.
    
    
    \item Set $\vp^{(t)}_i=\vp^{(t-1)}_i(1-\eta(\MA_i\vx^{(t)}-\vb_i))$ $\forall i\in \{1,..,2n+1\}$.\\ Set $\vp^{(t)}={\vp^{(t+1)}}/{{\lvert\lvert\vp^{(t+1)}\rvert\rvert}_1}$.
    
\end{enumerate}

At the end of $T$ iterations, the MWU algorithm returns $\vx={\sum\limits_{i=1}^T \vx^{(t)}}/{T}$ as the solution.

\paragraph{Justify correctness} Also argue how to recover discrete distribution from x. Argue size of obtained distribution.

\subsection{Implementing MWU}
\paragraph{Implementing Step (1)} Consider the expansion of the expression $\vp^T\MA\vx$. Observe that we can write it in the form $\sum\limits_{i=1}^{n} C_iz_{i}+\sum\limits_{p_j\in\P}D_jv_j$
where $C_i$ and $D_j$ are the respective coefficients of $u_i$ and $v_j$ in the expansion. Since the two terms do not share variables, we can maximize them independently. 
\par Observe that each $C_i=\vpos_i+\vpneg_i-{\vone}/{n}$. Hence, to maximize $\sum\limits_{i=1}^{n} C_iz_{i}$, we set each $z_i=1$ if $C_i\geq 0$, else we set $z_i=0$. 

\par To maximize $\sum\limits_{p_j\in\P}D_jv_j$, notice that by the Type \RNum{4} constraints $\sum\limits_{p_j\in\P}v_j\leq 1$. Hence, maximizing $\sum\limits_{p_j\in\P}D_jv_j$ depends only on the variable with the highest coefficient.
Let $j^*=\arg\max_j D_j $. If $D_{j^*}>0$, set $v_{j^*}=1$ and for all $j\neq j^{*}$, set $v_j=0$. Else, for all $j$, set $v_j=0$. 

\par The crux of the MWU is in implementing Step (1), once $x^{(t)}$ has been computed, Steps (2) and (3) are obvious and can be done in $O(n)$ time.


\paragraph{Running Time}. It is easy to see that maximizing $\sum\limits_{i=1}^{n} C_iz_{i}$ can be done in $O(n)$ time since each $z_i$ depends on exactly three constraints.  
\par Since each $D_j=\sum\limits_{R_i\cap p_j\neq\empty} (\vpos_j-\vpneg_j) $. Computing each $D_j$ takes $O(n)$ as we need to check the constraints corresponding to each range that contains $p_j$. 
Hence $v_{j^*}$ can be computed in $O(n^{d+1})$ time.
\subsection{Putting everything together}
In the previous sections we assumed that we know the value of $\opt$. In practice, we would need to guess it.

\par Let $\alpha \in [0,1]$ be a guess for the optimal error. Let $\eps=\frac{\delta}{16}$.
We discretize the range $[0,1]$ into a list of errors $E=\{\frac{\eps}{2}, (1+\eps)\frac{\eps}{2}, (1+\eps)^2\frac{\eps}{2},\ldots, 1\}$. We guess the optimal error $\alpha$ by running a binary search on $E$.
The algorithm starts with $\alpha$ set to the middle value of $E$ and tries to  find a distribution $\Dist'$ such that $\Error(\Dist',\TrainingSet)\leq \alpha+\eps$ using MWU. If the MWU aborts, it resets $\alpha$ to a larger value of $E$ following the binary search. If it succeeds, it resets $\alpha$ to a smaller value of $E$ following the binary search. In the end of the binary search, 
for a particular $\alpha$ that the MWU last succeeded, we get $\Dist'$. 
\newpage













\subsection{Algorithm}
Let $\alpha \in [0,1]$ be a guess for the optimal error. Let $\eps=\frac{\delta}{16}$.
We discretize the range $[0,1]$ into a list of errors $E=\{\frac{\eps}{2}, (1+\eps)\frac{\eps}{2}, (1+\eps)^2\frac{\eps}{2},\ldots, 1\}$. We guess the optimal error $\alpha$ by running a binary search on $E$.
The algorithm starts with $\alpha$ set to the middle value of $E$ and tries to  find a distribution $\Dist''$ such that $\Error(\Dist'',\TrainingSet)\leq \alpha+\eps$ using MWU.
If it fails, it resets $\alpha$ to a larger value of $E$ following the binary search. If it succeeds, it resets $\alpha$ to a smaller value of $E$ following the binary search. In the end of the binary search, 
for a particular $\alpha$ that the MWU last succeeded, we get $\Dist''$. The algorithm computes an $\eps$-approximation of $\Dist''$ and returns it as the output $\Dist'$.

%If it fails, it resets $\alpha:=\max(1,(1+\eps)\alpha)$ and restarts. For a particular $\alpha$, if the MWU concludes and outputs $\Dist''$, the algorithm computes an $\eps$-approximation of $\Dist''$ and returns it as the output $\Dist'$.
\par In a particular attempt at running MWU, the algorithm tries to iteratively solve the the following optimization problem:
%\paragraph{LP 1}
\begin{align*}
 \\
 \quad & \\
 & \frac{1}{n}\sum_{R_i\in\RangeSet} z_i\leq \alpha \quad \\
& z_i=|\sum_{p_j\in\P\cap R_i}v_j- s_i| \quad \forall R_i\in\RangeSet\\
& v_j\geq 0 \quad \forall p_j\in \P\\
& \sum_{p_j\in \P} v_j\leq 1 \\
& z_i\in [0,1] \quad \forall R_i\in \RangeSet
\end{align*}
The fact that the above optimization problem does not require the sum of the weights to be 1 is not of concern since it is trivial to find a point that lies outside $\RangeSet$ and assign it the remaining mass. Consider the following equivalent LP: 
 \paragraph{LP 2}
\begin{align*}
 \\
 \quad & \\
 & \sum_{R_i\in\RangeSet}-\frac{z_i}{n}\geq -\alpha \quad \text{(Type \RNum{1})} \\
& z_i+\sum_{p_j\in\P\cap R_i}v_j\geq s_i \quad \forall R_i\in\RangeSet \quad \text{(Type \RNum{2})}\\
&  z_i-\sum_{p_j\in\P\cap R_i}v_j\geq -s_i \quad \forall R_i\in\RangeSet \quad \text{(Type \RNum{3})}\\
& \sum_{p_j\in \P} v_j\leq 1 \quad \text{(Type \RNum{4})}\\
& v_j\geq 0 \quad \forall p_j\in \P \quad \text{(Type \RNum{4})}\\
& z_i\in [0,1] \quad \forall R_i\in \RangeSet \quad \text{(Type \RNum{4})}
\end{align*}
In any attempt, the MWU runs for $T=O(\frac{\ln(|\RangeSet|)}{\eps^2})$ iterations. Let $\F$ be a multi-set that is empty initially. In each iteration, the MWU process adds at most one point to $\F$. At the end of $T$ rounds, it returns the discrete distribution with support $\F$ where each point has weight $\frac{1}{T}$.\footnote{Note that the sum of weights of all points may be less than 1.}   Let $\MA\vx\geq \vb$ be the matrix-vector representation of the LP 2 ignoring the Type \RNum{4} constraints. Thus, $\MA$ is the constraint matrix, $\vx$ is the vector representing the variables, and $\vb$ is a vector representing the RHS of the constraints. The MWU algorithm maintains a probability vector $\vp$ whose dimension equals the number of rows of $\MA$. Thus $dim(\vp)=2|\RangeSet|+1$.
Let us denote the coordinate in $\vp$ with respect to the $j$-th Type \RNum{2} (resp. Type \RNum{3}) constraint by $\vpos_j$ (resp. $\vpneg_j$).
Let $Pos$ (resp. $Neg$) be the collection of coordinates of vector $\vp$ with respect to  Type \RNum{2} (resp. Type \RNum{3}) constraints.
%  Let $Pos$ (resp. $Neg$) be the collection of coordinates of the form $\vpos_j$ (resp. $\vpneg_j$).
Note that $|Pos|=|Neg|=|\RangeSet|$. Let $w(Pos)=\sum_{j\in Pos}\vpos_j$ (resp. $w(Neg)=\sum_{j\in Neg}\vpneg_j$) denote the sum of all values in $Pos$ (resp. $Neg$). Initially $\vp$ represents the uniform distribution. In each iteration $t$, the MWU algorithm checks if there exists a solution $\vx^{(t)}$ satisfying all Type \RNum{4} constraints such that $\vp^T\MA\vx^{(t)}\geq \vp^T\vb-\frac{\eps}{2}$ holds.

\paragraph{Checking Feasibility} Consider the expansion of the expression $\vp^T\MA\vx$. Observe that the LHS is of the form $\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{1}{n}C^{-}_i)z_{i}+\sum\limits_{p_j\in\P}(D^{+}_j-D^{-}_j)v_j$ where $C_i^{+}$ and $ D_j^{+}$ (resp. $C_i^{-}$ and $ D_j^{-}$) represent the sum of all positive (resp. negative) coefficients of each $z_i$ and $v_j$ in the expansion of $\vp^T\MA\vx$ respectively.

For any $i\leq |\RangeSet|$, we compute $C_i^+=\vpos_{i}+\vpneg_{i}$. Furthermore, $C_i^-=\vp_1$.
There is no non-trivial type \RNum{4} constraint for variables $z_i$, so for each $z_i^{(t)}$, set $z_i^{(t)}:=0$, if $(C^{+}_i-\frac{1}{n}C^{-}_i)\leq 0$, else set $z_i^{(t)}:=1$. Finally, we set $\gamma_1=\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{1}{n}C^{-}_i)z_{i}^{(t)}$. 


Next, we focus on setting the variables $v_j$, which is a more challenging task because the are $O(n^d)$ of them and there are non-trivial Type \RNum{4} constraints. 
We use an $\eps$-approximation schema to set the variables $v_j$ by (approximately) maximizing $\vp^T\MA\vx$.
We generate a subset of $S_1\subseteq \RangeSet$ by sampling $\kappa=O(\frac{1}{\eps^2}\log |\RangeSet|)$ rectangles where each rectangle $R_j$ is sampled with probability  $\frac{\vpos_j}{w(Pos)}$. Similarly, generate another subset $S_2\subseteq \RangeSet$ by sampling $\kappa$ rectangles where each rectangle $R_j$ is sampled with probability  $\frac{\vpneg_j}{w(Neg)}$. Let $\hat{S}=S_1\cup S_2$ be a weighted set of rectangles where each rectangle in $S_1$ has weight $\frac{w(Pos)}{\kappa}$ and each rectangle in $S_2$ has weight $-\frac{w(Neg)}{\kappa}$. Let $\square$ be the cell in $\Arr(\hat{S})$, the arrangement of $\hat{S}$, of maximum weighted depth. Take an arbitrary point $l_{\square}$ in $\square$.
\newcommand{\indx}{j^{l_\square}}
We find all rectangles in $\RangeSet$ that contain $l_\square$, so we can identify the index $\indx$ such that $p_{\indx}\in \P$ is contained in the same set of rectangles in $\RangeSet$ as the point $l_\square$.
We compute $D^{+}_{\indx}=\sum_{i: p_{\indx}\in R_i}\vpos_{i}$ and $D^{-}_{\indx}=\sum_{i: p_{\indx}\in R_i}\vpneg_{i}$.


If $\gamma+\max(0, (D^{+}_{\indx}-D^{-}_{\indx}))+\frac{\eps}{2}<\vp^T\vb$, declare that the current $\alpha$ is too small and abort the MWU. On the other hand, if $\gamma+max(0,(D^{+}_{\indx}-D^{-}_{\indx}))+\frac{\eps}{2}\geq \vp^T\vb$, then  if $D^{+}_{\indx}-D^{-}_{\indx}>0$, add $l_{\square}$ to $\F$.
%Let $v_{\indx}$ be the variable in LP 2 corresponding to the point $l_{\square}$.
If $(D^{+}_{\indx}-D^{-}_{\indx})>0$, consider $x^{(t)}$ to be the solution determined by setting each $z_i^{(t)}$ as above and ${v_{\indx}^{(t)}=1}$. Else, consider $x^{(t)}$ to be the solution determined by setting each $z_i^{(t)}$ as above and all $v_{\indx}^{(t)}=0$.

Next, the MWU requires to update each coordinate $\vp_j$ of $\vp$ such that ${\vp_j}^{(t+1)}:={\vp_j}^{(t)}\frac{(1-\eta (\MA_j\vx_j^{(t)}-b_j))}{\Phi^{(t)}} $. Depending on the constraint corresponding to $A_i$, the expression $(\MA_j\vx_j-b_j)$ can be determined from the computed values of each $z_i^{(t)}$ in the current iteration as well as checking if the rectangle corresponding to $\vp_j$ contains the point $l_{\square}$. Here $\eta=\frac{\eps}{12}$ and $\Phi^{(t)}$ is a normalizing constant to ensure $\vp$ remains a distribution. After updating $\vp$, the algorithm then moves on to the next iteration.



% Assign an integer label to each constraint in the above LP except for the last two constraints. The MWU algorithm maintains a non-negative weight $\beta_j$ for each constraint with label $j$. Note that there are $2|\RangeSet|+1$ such constraints. In the first iteration, $\forall j$,$B_j:=1$. In a particular iteration, the algorithm checks if the weighted sum of the contraints, where co 



\subsection{Analysis}
\paragraph{Correctness}  Suppose LP 2 has a feasible solution. Observe that for $\forall i\quad |\MA_i\vx-b_i|\in [-2,2]$. Therefore, by Theorem 3.5 of [AroraMWU], if in each iteration of the MWU, the algorithm can find a solution $\vx^{(t)}$ satisfying all Type \RNum{4} constraints such that $\vp^T\MA\vx^{(t)}\geq \vp^T\vb-\frac{\eps}{2}$ holds then after $T=O(\frac{\ln(|\RangeSet|)}{\eps^2})$ iterations, it is true that $\forall i\quad \MA_i\vx\geq \vb_i-\eps$ holds where $\vx=\frac{1}{T}\sum\limits_{t=1}^T \vx^{(t)}$. Assuming the algorithm checks feasibility in each iteration successfully, the description of the algorithm suggests that  $\vx=\frac{1}{T}\sum\limits_{t=1}^T \vx^{(t)}$ is equivalent to the discrete distribution with support $\F$ where each point has weight $\frac{1}{T}$. Because each $z_i$ may not capture the error of $R_i$ exactly, this implies $\Error(\Dist_{\F},\TrainingSet)\leq \Error(OPT,\TrainingSet)+3\eps$. Now it remains to prove that the algorithm can check feasibility in each iteration accurately. 

\par Observe that checking if there exists an $\vx$ such that $\vp^T\MA\vx \geq \vp^T\vb-\frac{\varepsilon}{2}$ under Type $\RNum{4}$ constraints is equivalent to maximizing $\vp^T\MA\vx$ under Type $\RNum{4}$ constraints. Recall that, $\vp^T\MA\vx=\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{1}{n}C^{-}_i)z_{i}+\sum\limits_{p_j\in\P}(D^{+}_j-D^{-}_j)v_j$. Furthermore, note that the two summations can be maximized independently because they do not have common variables. It is easy to verify that the algorithm maximizes $\sum\limits_{i=1}^{|\RangeSet|} (C^{+}_i-\frac{1}{n}C^{-}_i)z_{i}$.
For the term $\sum\limits_{p_j\in\P}(D^{+}_j-D^{+}_j)v_j$, observe that this is maximized by setting the variable with the largest coefficient to one if it is non-negative or else setting everything to zero. This is because $\sum\limits_{p_j\in \P} v_j\leq 1$. Let $v_{j^*}$ denote the variable with the largest coefficient. Recall $v_{\indx}$ is the variable found by the algorithm through the sampling step. 
\begin{lemma}
$(D^{+}_{\indx}-D^{-}_{\indx})\geq (D^{+}_{j^{*}}-D^{-}_{j^*})-\eps $
\end{lemma}
\begin{proof}
Consider the range space $\Sigma=(\Re^d,S_1)$ and its dual $\Sigma^D$. Since $|S_1|=\kappa=O(\frac{1}{\eps^2}\log |\RangeSet|)$, it is known that $S_1$ is an $\frac{\eps}{4}$-approximation for $\Sigma^D$ with probability at least $1-n^{O(d)}$. More specifically, it holds that  $|\frac{w_1(p_{j^*})}{\kappa}- \frac{D^{+}_{j^{*}}}{w(Pos)}|\leq \frac{\eps}{4}$, where $w_1(p_{j^*})$ denotes the  number of rectangles in $S_1$ containing $p_{j^*}$. Similarly, $S_2$ is is an $\frac{\eps}{4}$-approximation for $\Sigma^D$, so it holds that $|\frac{w_2(p_{j^*})}{\kappa}- \frac{D^{-}_{j^{*}}}{w(Neg)}|\leq \frac{\eps}{4}$, where $w_2(p_{j^*})$ denotes the  number of rectangles in $S_2$ containing $p_{j^*}$.
Equivalently, using the fact that $w(Pos)\in [0,1]$ and $w(Neg)\in [0,1]$, we can rewrite the inequalities above as,
$$D_{j^*}^+-\frac{\eps}{4}\leq w_1(p_{j^*})\frac{w(Pos)}{\kappa}\leq D_{j^*}^++\frac{\eps}{4}$$
$$D_{j^*}^--\frac{\eps}{4}\leq w_2(p_{j^*})\frac{w(Neg)}{\kappa}\leq D_{j^*}^-+\frac{\eps}{4},$$
so it follows that,
$$D_{j^*}^+-D_{j^*}^--\frac{\eps}{2}\leq w_1(p_{j^*})\frac{w(Pos)}{\kappa}-w_2(p_{j^*})\frac{w(Neg)}{\kappa}\leq D_{j^*}^+-D_{j^*}^-+\frac{\eps}{2}.$$
The same inequalities hold for any point in $\Re^d$, for example $l_\square$.
Recall that the algorithm chooses a point $l_\square$ in the cell $\square$ of $\Arr(\hat{S})$ with the maximum weighted depth.
By the inequalities above, it holds that,
$$D^{+}_{\indx}-D^{-}_{\indx}\geq w_1(l_\square)\frac{w(Pos)}{\kappa}-w_2(l_\square)\frac{w(Neg)}{\kappa}-\frac{\eps}{2}\geq w_1(p_{j^*})\frac{w(Pos)}{\kappa}-w_2(p_{j^*})\frac{w(Neg)}{\kappa}-\frac{\eps}{2}\geq D_{j^*}^+-D_{j^*}^--\eps.$$


%Together, they imply that for any point lying in a particular cell $\Delta$ of $\Arr(\hat{S}=S_1\cup S_2)$  (where each rectangle in $S_1$ has weight $\frac{w(Pos)}{\kappa}$ and each rectangle in $S_2$ has weight $-\frac{w(Neg)}{\kappa}$) the coefficient of its corresponding variable in $\vp^T\MA\vx$ is within $\frac{\eps}{4}$ of the weight of $\Delta$ in $\Arr(\hat{S})$. In particular this implies $v_{\indx}$ has coefficient at least $D^{+}_{j^{*}}-D^{-}_{j^{*}}-\frac{\eps}{2}$. 

\end{proof}

In any iteration of the MWU for $\alpha\geq \Error(OPT,\TrainingSet)$
%$\alpha\in [\max(\frac{\eps}{2}, \Error(OPT,\TrainingSet)),\max(\frac{\eps}{2}, (1+\eps)\Error(OPT,\TrainingSet))]$,
there exists a feasible solution, and therefore $max(0,D^{+}_{j^{*}}-D^{-}_{j^{*}})\geq\vp^T\vb-\gamma $. The above lemma implies $max(0,D^{+}_{j^{*}}-D^{-}_{j^{*}})-\max(0, (D^{+}_{\indx}-D^{-}_{\indx}) )\leq \frac{\eps}{2}$. Therefore, $\gamma+\max(0, w(l_{\square}))+\frac{\eps}{2}\geq \vp^T\vb$ must hold. This concludes the proof that the algorithm always finds a feasible solution when $\alpha$ in the above range.
\par Combining above along with the fact that the algorithm take an $\eps$-approximation (recall $\eps=\frac{\delta}{16}$)  at the end implies, $|\Dist'|\leq O(\frac{1}{\delta^2}\log\frac{1}{\delta})$ and $\Error(\Dist',\TrainingSet)\leq \Error(OPT,\TrainingSet)+\delta$ with high probability. 
\paragraph{Running Time}
The size of $E$ is $O(\frac{1}{\eps}\log\frac{1}{\eps})$ so the algorithm requires $O(\log\frac{1}{\eps}+\log\log\frac{1}{\eps})$ attempts.
%Since the algorithm starts with $\alpha=\frac{\eps}{2}$ and increases $\alpha$ by a factor of $(1+\eps)$ in each new attempt, it requires $O(\frac{1}{\eps}\log \frac{1}{\eps})$ attempts.
In each iteration of MWU, the coefficients of all the $z_i$ along with $\gamma$ can be computed in $O(n)$ time. Sampling $S_1$ and $S_2$ also require $O(n)$ time. Computing a point in the deepest cell of $\Arr(\hat{S})$ requires $f(|hat{S}|)=f(\frac{1}{\eps^2}\log |\RangeSet|)$.
Identifying the cell $p_{\indx}$ and computing the coefficient for the required $v_{\indx}$ variable takes $O(n)$ time. Each attempt of the MWU requires at most $\frac{1}{\eps^2}\log |\RangeSet|$ iterations. Since $\eps=\frac{\delta}{16}$, the overall running time is $O((\log\frac{1}{\delta}+\log\log \frac{1}{\delta})(n+f(\frac{1}{\delta^2}\log^{\frac{d}{2}} |\RangeSet|))\frac{1}{\delta^2}\log |\RangeSet|)$.

If $\RangeSet$ consists of a set of rectangles then the deepest cell of $\Arr(\hat{S})$ can be computed in
$\Tilde{O}(|\hat{S}|^{d/2})=\Tilde{O}(\frac{1}{\eps^d}\log^{\frac{d}{2}} |\RangeSet|)$ time using standard techniques \cite{oy-nubkm-91}. The overall running time is $\Tilde{O}((\log\frac{1}{\delta}+\log\log \frac{1}{\delta})(n+\frac{1}{\delta^d}\log^{\frac{d}{2}} |\RangeSet|)\frac{1}{\delta^2}\log |\RangeSet|)=\tilde{O}(\frac{n}{\delta^2}+\frac{1}{\delta^{d+2}})$.

==> backupProof.tex <==
We compute a deepest point $\tilde{p}^{(t)}_h$ with respect to $(\epsApprox_h,\bar{\omega})$ by calling $\algDeep(\epsApprox_h,\bar{\omega})$.
After repeating $\mu$ times, we choose as $\tilde{p}^{(t)}$
the point $\tilde{p}_h^{(t)}$ that maximizes $\depth(\tilde{p}^{(t)}_h,\RangeSet,\vomega)$.
%$=\max_{1\leq h\leq \mu}\depth(\tilde{p}^{(t)}_h,\epsApprox_h,\bar{\vomega})$.
Recall that $\vomega^{(t)}_i=w^{(t)}_{2i}-w^{(t)}_{2i-1}$.
\begin{lemma}
\label{lem:deepestpoint}
$\depth(\tilde{p}^{(t)},\RangeSet,\omega^{(t)})\geq \max_{x\in \Re^d}\depth(x,\RangeSet, \omega^{(t)})-\delta/12$ with probability at least $1-1/n^{O(1)}$.
\end{lemma}
\begin{proof}
Set $\bar{\delta}=\delta/48$.
If we choose the constant $c_3$ sufficiently large, then both $\epsApprox_h^+$ and $\epsApprox_h^-$ are $\bar{\delta}$-approximations with probability at least $1/2$.
Therefore, for any point $x\in \Re^d$,
\begin{equation}
\label{eq:epsApproxProof}
\cardin{\frac{\depth(x,\RangeSet,\vp^+)}{\norm{\vp^+}_1}-\frac{\depth(x,\epsApprox^+_h)}{\cardin{\epsApprox^+_h}}}, \cardin{\frac{\depth(x,\RangeSet,\vp^-)}{\norm{\vp^-}_1}-\frac{\depth(x,\epsApprox^-_h)}{\cardin{\epsApprox^-_h}}}\leq \delta/48.
\end{equation}
Using~\eqref{eq:epsApproxProof} and the fact that $\norm{\vp^+}_1, \norm{\vp^-}_1\leq 1$, we obtain 
\begin{align*}
\depth(x,\RangeSet,\vomega^{(t)})&=\depth(x,\RangeSet,\vp^+)-\depth(x,\RangeSet,\vp^-)\\
&\leq \frac{\norm{\vp^+}_1}{r}\depth(x,\epsApprox_h^+)-\frac{\norm{\vp^-}_1}{r}\depth(x,\epsApprox_h^-)+2\frac{\delta}{48}\\
&=\depth(x,\epsApprox_h,\bar{\vomega})+\frac{\delta}{24}.
\end{align*}
Similarly, $$\depth(x,\RangeSet,\vomega^{(t)})\geq \depth(x,\epsApprox_h,\bar{\vomega})-\frac{\delta}{24}.$$
Let $x^*=\argmax_{x\in \Re^d}\depth(x,\RangeSet,\vomega^{(t)})$.
Hence, $\depth(\tilde{p}^{(t)}_h,\RangeSet, \vomega^{(t)})\geq \depth(x^*,\RangeSet, \vomega^{(t)})-\delta/12$, with probability at least $1/2$.
We repeat the algorithm $O(\log n)$ iterations, so with probability at least $1-1/n^{O(1)}$,
$$\depth(\tilde{p}^{(t)},\RangeSet,\vomega^{(t)})\geq \depth(x^*,\RangeSet,\vomega^{(t)})-\frac{\delta}{12}.$$

==> backupProof2.tex <==
We compute a deepest point $\tilde{p}^{(t)}_h$ with respect to $(\epsApprox_h,\bar{\omega})$ by calling $\algDeep(\epsApprox_h,\bar{\omega})$.
After repeating $\mu$ times, we choose as $\tilde{p}^{(t)}$
the point $\tilde{p}_h^{(t)}$ that maximizes $\depth(\tilde{p}^{(t)}_h,\hat{\epsApprox},\hat{\vomega})$, where $\hat{\epsApprox}, \hat{\vomega}$ are defined as follows.
$\hat{\epsApprox}$ is the union of a random sample $\hat{\epsApprox}^+$ of $(\RangeSet, \vp^+)$ and 
a random sample $\hat{\epsApprox}^-$ of $(\RangeSet, \vp^-)$ of size $\hat{r}=c_4\delta^{-2}\log n$, each.
The weight function
$\hat{\vomega}:\hat{\epsApprox}\rightarrow\Re$ is defined similarly to $\bar{\vomega}$ replacing $r$ with $\hat{r}$. Notice that $\hat{\epsApprox}$ is built only once. By definition, each $\epsApprox_h$ is an $O(\delta)$-approximation with constant probability, while the $\hat{\epsApprox}$ is an $O(\delta)$-approximation with high probability.
Recall that $\vomega^{(t)}_i=w^{(t)}_{2i}-w^{(t)}_{2i-1}$.
\begin{lemma}
\label{lem:deepestpoint}
$\depth(\tilde{p}^{(t)},\RangeSet,\omega^{(t)})\geq \max_{x\in \Re^d}\depth(x,\RangeSet, \omega^{(t)})-\delta/12$ with probability at least $1-1/n^{O(1)}$.
\end{lemma}
\begin{proof}
If we choose the constant $c_3$ sufficiently large, then both $\epsApprox_h^+$ and $\epsApprox_h^-$ are $\frac{\delta}{96}$-approximations with probability at least $1/2$.
Therefore, for any point $x\in \Re^d$,
\begin{equation}
\label{eq:epsApproxProof}
\cardin{\frac{\depth(x,\RangeSet,\vp^+)}{\norm{\vp^+}_1}-\frac{\depth(x,\epsApprox^+_h)}{\cardin{\epsApprox^+_h}}}, \cardin{\frac{\depth(x,\RangeSet,\vp^-)}{\norm{\vp^-}_1}-\frac{\depth(x,\epsApprox^-_h)}{\cardin{\epsApprox^-_h}}}\leq \delta/96.
\end{equation}
Using~\eqref{eq:epsApproxProof} and the fact that $\norm{\vp^+}_1, \norm{\vp^-}_1\leq 1$, we obtain 
\begin{align*}
\depth(x,\RangeSet,\vomega^{(t)})&=\depth(x,\RangeSet,\vp^+)-\depth(x,\RangeSet,\vp^-)\\
&\leq \frac{\norm{\vp^+}_1}{r}\depth(x,\epsApprox_h^+)-\frac{\norm{\vp^-}_1}{r}\depth(x,\epsApprox_h^-)+2\frac{\delta}{96}\\
&=\depth(x,\epsApprox_h,\bar{\vomega})+\frac{\delta}{48}.
\end{align*}
Similarly, $$\depth(x,\RangeSet,\vomega^{(t)})\geq \depth(x,\epsApprox_h,\bar{\vomega})-\frac{\delta}{48}.$$
Let $x^*=\argmax_{x\in \Re^d}\depth(x,\RangeSet,\vomega^{(t)})$.
Hence, $\depth(\tilde{p}^{(t)}_h,\RangeSet, \vomega^{(t)})\geq \depth(x^*,\RangeSet, \vomega^{(t)})-\delta/24$, with probability at least $1/2$.
We repeat the algorithm $O(\log n)$ iterations, so with probability at least $1-1/n^{O(1)}$,
there exists $h^*\in[1,\mu]$ such that 
$$\depth(\tilde{p}_{h^*}^{(t)},\RangeSet,\vomega^{(t)})\geq \depth(x^*,\RangeSet,\vomega^{(t)})-\frac{\delta}{24}.$$

Next, we note that for sufficiently large constant $c_4$, the sample $\hat{\epsApprox}$ is a $\frac{\delta}{96}$-approximation of $(\RangeSet, \vomega^{(t)})$ with probability at least $1-1/n^{O(1)}$.
Hence, with high probability, we have 
\begin{align*}
\depth(\tilde{p}^{(t)},\RangeSet,\vomega^{(t)})&\geq \depth(\tilde{p}^{(t)},\hat{\epsApprox},\hat{\vomega})-\frac{\delta}{48}\geq \depth(\tilde{p}_{h^*}^{(t)},\hat{\epsApprox},\hat{\vomega})-\frac{\delta}{48}\\
&\geq\depth(\tilde{p}_{h^*}^{(t)},\RangeSet,\vomega^{(t)})-\frac{\delta}{24}\geq \depth(x^*,\RangeSet,\vomega^{(t)})-\frac{\delta}{12}.
\end{align*}
\end{proof}

==> prelims.tex <==
\section{Preliminaries:}
% \subsection{Multiplicative Weighted Update method}
% \label{subsec:MWU}
% In this work we use the Multiplicative Weighted Update (MWU) method to prove the correctness of our new algorithms. In particular, we use the results in~\cite{arora2012multiplicative}. The goal is to solve the following feasibility problem. Given a convex set $\mathcal{P}$ in $\Re^n$ and concave functions $f_i:\mathcal{P}\rightarrow \Re$ for $i\in[1,m]$, return (if there exists) a vector $x\in \mathcal{P}$ such that $f_i(x)\geq 0$ for each $i\in [1, n]$.
% They define a general method that works in iterations. More specifically, in every iteration, given a probability vector $\vp=(\vp_1,\ldots, \vp_m)$ (in the first iteration each $\vp=\frac{1}{m}$), assume that there exists an oracle for the following simpler feasibility problem: We want to find $x\in \mathcal{P}$ (if there exists one) such that $\sum_i \vp_i \cdot f_i(x)\geq -\eps/3$. Let $x^{(j)}$ be the solution to the oracle. The oracle is called $(\ell,\rho)$-bounded if $-\ell\leq f_i(x^{(j)})\leq \rho$ for each $i\in [1,m]$. Base on the error $f_i(x^{(j)})$ of each constraint in the original problem, the MWU method updates the vector probability $\vp$ and run the same procedure. The algorithm runs for $T=O(\ell\rho\log(m)/\eps^2)$ and in the end, if all oracles are feasible, it returns $\bar{x}=\frac{1}{T}\sum_{j=1}^T x^{(j)}$ as the final solution. They prove that $f_i(\bar{x})\geq -\eps$ for each $i\in [1,m]$.
% Overall, they prove the next theorem.
% \begin{theorem}[\cite{arora2012multiplicative}]
% \label{thm:MWU}
% Let $\eps$ be a given error parameter. Suppose there exists an $(\ell,\rho)$-bounded oracle. Assume that $\ell\geq \eps/3$. Then there is an algorithm which either solves the feasibility problem up to an additive error of $\eps$, or correctly concludes that the system is infeasible, making only $O(\ell\rho\log(m)/\eps^2)$ calls to the oracle, with an additional processing time of $O(m)$ per call.
% \end{theorem}
% % 2. epsilon-nets
% % 3. epsilon-approximations
% % 4. Range Spaces
% % 5. Range Trees
% % \\\\\\








==> temp.tex <==
\section{Temporary: Ignore}

\paragraph{Updated Sampling Scheme} 
Let $Pos$ (resp. $Neg$) be the collection of coordinates of $\vp$ of the form $\vpos_j$ (resp. $\vpneg_j$).
Note that $|Pos|=|Neg|=|\RangeSet|$. Let $w(Pos)=\sum_{j\in Pos}\vpos_j$ (resp. $w(Neg)=\sum_{j\in Neg}\vpneg_j$) denote the sum of all values in $Pos$ (resp. $Neg$). 
\par 

Generate a sample of $S_1\subseteq \RangeSet$ by sampling $\kappa=O(\frac{1}{\eps^2}\log n)$ rectangles where each rectangle $R_j$ is sampled with probability  $\frac{\vpos_j}{w(Pos)}$. Similarly, generate another subset $S_2\subseteq \RangeSet$ by sampling $\kappa$ rectangles where each rectangle $R_j$ is sampled with probability  $\frac{\vpneg_j}{w(Neg)}$. 
       
        Let $\hat{S}=S_1\cup S_2$ be the weighted set (possibly multi-set) of rectangles. Let $w:\hat{S}\rightarrow \Re$ be a weight function such that $w(s)=\frac{w(Pos)}{\kappa}$ if $s\in S_1$ else $w(s)=-\frac{w(Neg)}{\kappa}$. Build a weighted range tree on $\hat{S}$. 

    \par Repeat the following for $O(\log n)$ steps:

    Sample two sets $\bar{S_1}$ and $\bar{S_2}$ from $\RangeSet$ each of size $\eta=\frac{1}{\eps^2}\log \frac{1}{\eps^2}$  where the sampling is done proportional to $Pos$ and $Neg$ respectively as above.
    Set weights as above.  Run $\deep(\hat{S},w)$ to find the deepest point $\bar{p}$ with respect to $(\hat{S},w)$. Use range data structure from above to check weight of $\Bar{p}$.
